EventFull: Complete and Consistent Event Relation Annotation

Event relation detection is a fundamental NLP task, leveraged in many downstream applications, whose modeling requires datasets annotated with event relations of various types. However, systematic and complete annotation of these relations is costly and challenging, due to the quadratic number of event pairs that need to be considered. Consequently, many current event relation datasets lack systematicity and completeness. In response, we introduce \textit{EventFull}, the first tool that supports consistent, complete and efficient annotation of temporal, causal and coreference relations via a unified and synergetic process. A pilot study demonstrates that EventFull accelerates and simplifies the annotation process while yielding high inter-annotator agreement.

==> backup/background_last.tex <==
\section{Background and Related Work}
This section overviews relevant research on event graphs, covering event-event relation types (\S\ref{back:event-rels}), the desired properties of such graphs (\S\ref{back:compl-consist-complex}), annotation schemes (\S\ref{back:annot-schemes}) and tools (\S\ref{back:annot-tools}).

\subsection{Event-Event Relations}
\label{back:event-rels}
The three main relations types considered by \App{} are: \textbf{Temporal}, for understanding the sequence of events over time \cite{do-etal-2012-joint}; \textbf{Causal}, for understanding how one event influences another in a story \cite{chaturvedi-etal-2017-story}; and \textbf{Coreference}, for identifying mentions of the same event in texts \cite{raghunathan-etal-2010-multi}.\footnote{An additional relation type often considered is the sub-event relation \cite{glavas-etal-2014-hieve}. However, it is beyond the scope of this work.} Importantly, the latter two relations are directly governed by the temporal relation, i.e., coreferring events occur at the same time and events that cause other events naturally occur before them.

%The coreference and causal relations are constrained by the temporal relation. Event mentions that corefer must be identical in time and duration. For an event to cause another, it must start \emph{before} the affected event.


\subsection{Completeness and Consistency}
\label{back:compl-consist-complex}
To create a high-quality and exhaustive event relation graph, it is crucial to monitor annotation \emph{completeness} and \emph{consistency} \cite{marc-et-al-2005-temporal}, ensuring that each type of relation exists between any pair of events, and there are no relations that contradict each other—either directly and transitively, or between relation types (e.g., a causing event occurring \emph{after} the affected event). 

Previous works did not always account for these attributes. For instance, in the notable TimeBank corpus \cite{pustejovsky-etal-2003}. \citet{pustejovsky-stubbs-2011-increasing} identified inconsistencies, and \citet{reimers-etal-2016-temporal} criticized it for missing many relations. Similarly, in our experiments, we discovered a few inconsistencies in the TCR \cite{ning-etal-2018-joint} and EventCausality \cite{do-etal-2011-minimally} datasets across relation types (such as \emph{cause/after}). One of our primary goals in developing \App{} is to ensure that the produced event relation graph is consistent and complete.


%by identifying all pairs of events that require annotation and preventing contradictions in direct, transitive, and across different types of relations (for example, a \emph{cause} must align with a \emph{before} temporal relation). (2) Reducing annotation \emph{complexity} to make the process feasible and manageable for annotators.

% To that end \App{} is integrated with a framework that enforce these attributes, as further detailed in §\ref{tool:logic}.



\subsection{Annotation Schemes}
\label{back:annot-schemes}
Several previous studies have proposed different annotation schemes for each of the aforementioned event-event relations.

\paragraph{Temporal} 
All prior related work, including RED, EventStoryLine \cite{caselli-vossen-2017-event}, and MAVEN-ERE \cite{wang-etal-2022-maven}, was annotated following the TimeML \cite{pustejovsky2003timeml} annotation scheme. This scheme considers all events in a document and requires the anchoring of events to explicit time expressions (i.e., TimeX\footnote{Temporal expression mark-up for temporal entities} or the DCT\footnote{The document creation time}) to establish temporal relations. %Thus, an event that cannot be anchored to any explicit time expression in the text is not annotated. 
However, time expressions are not always present, as writers focus on advancing their story in an engaging way rather than detailing every aspect. 
%Readers can either infer the relation using common-sense reasoning, or in some cases, the relation is indeterminate from the text and should be marked as vague (indicating that it was investigated but could not be resolved). 
Consequently, the TimeML approach does not consider (by design) all temporal relations between all pairs of events \cite{cassidy-etal-2014-annotation, rogers2022narrativetime}.

Our goal is to develop a tool that supports exhaustive annotation of event-event relations, and for this purpose, we have adopted the novel Multi-Axis annotation scheme \cite{ning-etal-2018-multi}. This method streamlines the process by focusing only on actual events, excluding hypothetical or intentional ones, and considers only four relation types: before, after, equal, and vague, focusing solely on event start times. These simplifications help achieve high agreement among annotators. To determine the relationship between two events, A and B, annotators answer two yes/no questions: A1) if A started before B, and A2) if B started before A. Then map the answer as follows: A1=A2=yes$\rightarrow$vague, A1=A2=no$\rightarrow$equal, A1=yes, A2=no$\rightarrow$before, and A1=no, A2=yes$\rightarrow$after.

%in three key ways: (1) Four types of temporal relations are considered: \emph{before}, \emph{after}, \emph{equal}, and \emph{uncertain}, as opposed to the seven TimeML relations. 
%This reduction includes the most critical temporal relations and provides the necessary framework for annotating coreference and causal relations, which are temporally constrained by the \emph{equal} and \emph{before/after} relations. 
%(2) Events are categorized into logical timeline \emph{axes} (as listed in step 1 of Figure~\ref{fig:figure1}), distinguishing actual events (main axis) from theoretical ones (other axes). Since establishing a timeline between events that occurred and those that did not is impractical, temporal relations are permitted only between events on the same axis. (3) Only the starting time of events is considered. 

%Overall, these simplifications helped achieve high agreement among annotators. Consequently, we have adopted this method in our tool (§\ref{tool}).
%To the best of our knowledge, \App{} is the first annotation tool to support this annotation methodology.
%previous temporal annotation tools adhere to the TimeML scheme \cite{cassidy-etal-2014-annotation, derczynski-etal-2016-gate, fulda-etal-2016}, while no existing tools follow the Multi-Axis guidelines.

While this approach supports our goal, annotating relations between all \textit{actual} events remains complex. We developed \App{} to help reduce this complexity, as detailed in §\ref{tool:temp}.

%is considered not feasible, due to the quadruple complexity challenge. In an attempt to address this and increase the density of temporal relations, various studies \cite{cassidy-etal-2014-annotation, minard-etal-2016-meantime, caselli-vossen-2017-event, ning-etal-2018-joint} annotated relations only between adjacent sentences.


\paragraph{Coreference} For the coreference annotation, our tool adheres to the traditional coreference chains annotation methodology \cite{cybulska-vossen-2014-using, ogorman-etal-2016-richer}. In this approach, annotators cluster event mentions that refer to the same real-world event into coreference clusters. Event mentions that do not corefer with other mentions are marked as singleton clusters.


\paragraph{Causal} For causal relations, it is common practice to use the RED annotation scheme \cite{ogorman-etal-2016-richer}, which requires annotators to assess if \emph{the tail event is inevitable given the head event}. This approach, however, involves evaluating every pair of event mentions, posing a significant challenge in terms of complexity.

Since our approach aims to reduce the quadruple annotation complexity necessary for achieving a complete event graph. We have adopted the EventStoryLine methodology \cite{caselli-vossen-2017-event},\footnote{We focus solely on the causal relation (excluding enablement), similar to \citet{ning-etal-2018-joint, do-etal-2011-minimally}.} In contrast to RED, this methodology presents each tail event alongside \emph{all} preceding events. Annotators are tasked with determining \emph{why the tail event occurred} and identifying if the cause is among the listed candidates (head events). Our experiments (detailed in §\ref{app:cause-scheme-expr}) demonstrate that this method is more efficient and achieves higher agreement among annotators. 

%In contrast, the EventStoryLine methodology \cite{caselli-vossen-2017-event} presents each tail event alongside all preceding events. Annotators are tasked with determining \emph{why the tail event occurred} and identifying if the cause is among the listed candidates. Our experiments (detailed in §\ref{tool:logic}) demonstrate that this method is more efficient and achieves higher agreement among annotators. Therefore, we have adopted the EventStoryLine approach in \App{}.\footnote{We only consider the causal relation (without enablement), similar to \citet{ning-etal-2018-joint, do-etal-2011-minimally}.}

%For the causal annotation, we adopt the annotation methodology from EventStoryLine \cite{caselli-vossen-2017-event},\footnote{We only consider the causal relation (without enablement), similar to \citet{ning-etal-2018-joint, do-etal-2011-minimally}.} where each tail event is presented with all preceding events. The annotator needs to determine \emph{why the tail event has happened} and then verify if the causing event is among the listed candidates. This in contrast to the RED \cite{ogorman-etal-2016-richer} annotation methodology, where given an event pair, involves assessing if \emph{the tail event is inevitable given the head event}. We further discuses our motivation for adopting the EventStoryLine methodology in §\ref{tool:logic}.

\subsection{Existing Annotation Tools}
\label{back:annot-tools}

%Existing datasets that encompass the temporal, coreference and causal relations (or a subset of these relations) \cite{chaturvedi-etal-2017-story, mirza-etal-2014-annotating, hong-etal-2016-building, ogorman-etal-2016-richer, wang-etal-2022-maven}, have either utilized and customized general-purpose tools such as BRAT \cite{stenetorp-etal-2012-brat} or CAT \cite{bartalesi-lenzi-etal-2012-cat}, or did not release or specify the use of any annotation tool.

Currently, to establish an event-event relation annotation that encompasses multiple relations, two options are available: (1) using general-purpose annotation tools like BRAT \cite{stenetorp-etal-2012-brat} and CAT \cite{bartalesi-lenzi-etal-2012-cat}, which offer extensive customization features and comprehensive administrative capabilities. 
However, they lack specific implementations crucial for managing the complexity of exhaustive annotations and ensuring completeness and consistency. (2) using several annotation tools, each dedicated to a specific type of relation. Yet, all temporal annotation tools \cite{cassidy-etal-2014-annotation, derczynski-etal-2016-gate, fulda-etal-2016, rogers2022narrativetime} follow the TimeML annotation scheme, and no existing tool supports causal annotation. Furthermore, using multiple tools to annotate different types of relations poses significant challenges in terms of handling and maintenance.

% To the best of our knowledge, \App{} is the first annotation tool to support end-to-end annotation of temporal, causal, and coreference relations, enforcing completeness and consistency while managing complexity (further detailed in §\ref{tool}).

% In the individual relation annotation space, a variety of tools have been developed over the years for specific tasks, such as temporal relation annotation \cite{verhagen-etal-2006-annotation, verhagen-pustejovsky-2008-temporal, cassidy-etal-2014-annotation, derczynski-etal-2016-gate, fulda-etal-2016, rogers2022narrativetime}, and coreference \cite{girardi-etal-2014-cromer, oberle-2018-sacr, bornstein-etal-2020-corefi}.\footnote{To the best of our knowledge, no tool exists specifically for annotating causal relations.} However, most temporal annotation tools adhere to the TimeML scheme. Additionally, using multiple tools to annotate different types of relations poses significant challenges in terms of handling and maintenance.



==> backup/background_text.tex <==

%This sparsity subsequently impact the density of causal and coreference relations, as those are temporally constrained (where annotators consider pairs of events with an \emph{equal} time relation for the coreference and \emph{before/after} time relation for the causal).


%Furthermore, while temporal relations inherently exist between any pair of events, allowing us to disregard unjudged event pairs when training or testing a model, causal and coreference relations might not exist between events. Thus, incompletely annotated causal and coreference relations might cause unjudged pairs to mistakenly be considered as negative examples.

% In this section, we first review the multi-axis annotation scheme (§\ref{back:multi}) which we followed for the temporal relation annotation. We then review event relation extraction tools that support the annotation of event-event relations (§\ref{back:annot-tools}). 


% \subsection{Multi-Axis Scheme}
% \label{back:multi}

% %\footnote{This scheme was fully or partially adopted in several recent works \cite{ning-etal-2018-multi, ning-etal-2018-joint, wang-etal-2022-maven}} 

% Using this annotation scheme, subsequent works \cite{ning-etal-2018-multi, ning-etal-2018-joint, wang-etal-2022-maven} achieved relatively high inter-annotator agreement (above 0.7 Cohen’s Kappa). To ensure high agreement and facilitate the exhaustive annotation of temporal relations between events, we adopted this scheme in our tool.


% \subsection{Existing Annotation Tools}
% \label{back:annot-tools}
% \avivs{Shouldn't this section be related work? and then we can also elaborate on the different relations - e.g., causal, temporal, etc.}
% \avivs{I wouldn't start with "To the best of our knowledge, there is currently no tool..." but rather first list all the things that do exist, and only in the end say that no such tool exists.}

%This leaves the heavy lifting—such as selecting pairs of events to annotate, ensuring all events are covered, skipping event relations that might be inferred transitively, and avoiding contradicting events—up to the annotator or task administrator.

%Consequently, previous research often depended on general-purpose, highly customizable tools such as BRAT \cite{stenetorp-etal-2012-brat} and CAT \cite{bartalesi-lenzi-etal-2012-cat}. Yet, BRAT and CAT are not specifically tailored for event-event relation annotation and do not sufficiently ensure annotation completeness (ensuring all required relations are annotated), consistency (avoiding contradictory annotations), or help in reducing the annotation complexity.

%However, The Brat tool is designed to provide custom configuration for annotating any relation between text entities, however it does not provide any specific annotation aid for the type of annotation required to facilitate the event relation annotation. Similarly, CAT while provides some specific implementation for the TimeML annotation scheme \cite{pustejovsky2003timeml}, it does not provide much beyond to help annotate temporal relations to insure completeness and consistence or support for any of the other relations. Thus, Brat and Cat does not mitigate the quadruple annotation complexity, or insure annotation completeness and consistency, which will probably result in high annotation effort and low IAA.

%Due to those limitations, other dataset authors developed their own proprietary tools (\alone{cite Causal-TB, EER}) for their annotation, however they did not release those tools for future work. The rest of the datasets authors in this domain did not indicate using any annotation tools (\alone{cite RED, MAVEN-ERE}).

%\avivs{in the background - discuss the annotation scheme and annotation tool and for the different objectives of our work (exhaustiveness).}

%, addressing two of the main challenges faced in the field of event-event relation annotation (\aeirew{find and cite the paper}).

%Since a low IAA, the community has been looking into ways to simplify the task, by reducing the label set, and by breaking up the overall, complex task into subtasks (e.g., getting agreement on which event pairs should have a relation, and then what that relation should be) (Mostafazadeh et al., 2016; O’Gorman et al., 2016). In contrast to other existing datasets, Bethard et al. (2007) achieved an agreement as high as 90\%, but the scope of its annotation was narrowed down to a very special verb-clause structure.


% \subsection{Event-Event Relations}
% \label{back:coref-cause-temp}
% Our tool focuses on facilitating the annotating of three key event-event relations: temporal, causal, and coreference. 

% The \emph{coreference} relation indicates whether two events mentioned in text are in fact two mentions of the same real world event. This inherently implies that coreferring event mentions share identical (i.e., coreferring) arguments, notably the same time. 


% The \emph{causal} relation is centered around identifying whether one event \emph{caused} another event to occur. Like the coreference relation, the causal relation is also bound by temporal constraints. Specifically, if event $A$ causes event $B$, it naturally implies that event $A$ started before event $B$. 


%There are two primary types of causality relations in the literature; causal and precondition. Precondition means that if event A occurred, it enabled event B to occur, however it did not cause it (e.g., \emph{connecting} to a Wi-Fi enabled me to \emph{login} to my account), and causality means that if event A occurred, event B most definitely occurred as well (e.g., the \emph{earthquake} caused \emph{damage}). In both cases, event A started before event B, and the in-occurrence of event A \emph{prevents} event B from triggering. To that end, in this work we adopted the more inclusive case of precondition as the causal relation, following (\alone{cite Causal-TB, TCR and EventCausality}) we adopted the C-Link relation (\alone{cite Causal-TB?}) in our causal annotation scheme. 

% The \emph{temporal} relations contribute to understanding the temporal ordering of events. Various annotation schemes have been developed to address different levels of granularity in temporal relations, ranging from 13 to 4 temporal relations categories \cite{ogorman-etal-2016-richer, pustejovsky2003timeml, ALLEN1984123, mostafazadeh-etal-2016-caters, ning-etal-2018-multi}. 



%However, this method does not address the quadruple complexity, nor does it ensure the completeness and consistency of annotating temporal relations. Our work aims to extend beyond these limitations by addressing these crucial aspects.

%\footnote{Though \citet{ning-etal-2018-multi} focuses exclusively on temporal relations, the restriction implicitly extends to other types of relations as well.} These include the \emph{main} axis for actual events that have occurred (in past or present) or planned to occur, the intentional axis for events that are planned but have not yet occurred, and the hypothetical axis for events that might or might not occur. This reduce situations where annotators are presented with events that cannot logically share a relation, and potentially improve the Inter-Annotator Agreement (IAA).
% (3) Observing that annotators struggle in determining the end time of events, which consequently reduce IAA, and since specifying the end time is not essential for the four mentioned relations, the multi-axis method only consider the starting time of events. However, this method does not address the quadruple complexity, nor does it ensure the completeness and consistency of annotating temporal relations. Our work aims to extend beyond these limitations by addressing these crucial aspects.

%Additionally, while causal and coreference relations are annotated in isolation (a pair of events cannot simultaneously corefer and cause one another), temporal relations coexist alongside them. Thus, understanding the temporal relationship between events can be crucial in determining whether a pair of events should be further investigated for potential causal or coreference relations \cite{wang-etal-2022-maven}. 

% Considering the complexity in annotating many types of temporal relations, and the fact that causal and coreference relations are constrained only by `before' and `equal' temporal relations, our work adopts the innovative multi-axis \cite{ning-etal-2018-multi} annotation scheme.\footnote{This scheme was fully or partially adopted in several recent works \cite{ning-etal-2018-multi, ning-etal-2018-joint, wang-etal-2022-maven}} This approach simplifies temporal annotation in three key ways: 
% (1) Only four types of temporal relations are considered: \emph{before}, \emph{after}, \emph{equal}, and \emph{vague}, thus, it encompasses the most critical temporal relations and the necessary relations for the coreference and causal relations.
% (2) Events are divided into theoretical timeline axes, where relations are permissible only within the same axis.\footnote{Though \citet{ning-etal-2018-multi} focuses exclusively on temporal relations, the restriction implicitly extends to other types of relations as well.} These include the \emph{main} axis for actual events that have occurred (in past or present) or planned to occur, the intentional axis for events that are planned but have not yet occurred, and the hypothetical axis for events that might or might not occur. This reduce situations where annotators are presented with events that cannot logically share a relation, and potentially improve the Inter-Annotator Agreement (IAA).
% (3) Observing that annotators struggle in determining the end time of events, which consequently reduce IAA, and since specifying the end time is not essential for the four mentioned relations, the multi-axis method only consider the starting time of events. However, this method does not address the quadruple complexity, nor does it ensure the completeness and consistency of annotating temporal relations. Our work aims to extend beyond these limitations by addressing these crucial aspects.

% Additionally, our annotation scheme draws inspiration from \cite{wang-etal-2022-maven}. In their manual annotation process, the authors presented annotators with only the logical relations to consider during the coreference and causal annotation steps—specifically, 'equal' relations for coreference and 'before/after' relations for cause/effect. It is noteworthy that equal relations comprise on average 1-3\% of all relations \cite{chambers-etal-2014-dense, wang-etal-2022-maven}, significantly reducing coreference annotation complexity. Although 'before' and 'after' relations are more prevalent, selectively presenting only these relations to annotators reduces the complexity involved in annotating causal relationships.

%\footnote{Notably, the coreference relation does require the end time to be established, however this is deducted if at the coreference annotation step the annotator make the decision regarding whether two events with equal relation corefere}

%Applying this scheme have assisted the authors of MATRES in reducing annotation complexity, enabling the use of non-expert annotators while still achieving a relatively high IAA. 


%\subsection{Transitive Closure}
% \label{back:tmp-trans-clos}
% Deducing the transitive relation in a temporal graph is a challenging task that was explored in the interval algebra of \cite{allen-et-al-1983}, the point algebra of \cite{VILAIN1990373} and in TimeML \cite{pustejovsky2003timeml}. Since our annotation scheme follow a more narrow scheme covering a subset of four temporal relations (after, before, equal, vague), we developed a transitive closure algorithm inspired by \cite{ALLEN1984123, VILAIN1990373, setzer-2002-temp, pustejovsky2003timeml}, specific to our temporal annotation scheme and further extended it to support both annotation completeness and consistency in the annotation steps of all relations (further explained in §\ref{tool:logic}).


%can only depends on comparing the begging time of events for the equal, before, and after relations. In this work we follow the novel multi-axis \cite{ning-etal-2018-multi} annotation scheme, which simplify temporal annotation in three main aspects: (1) dividing events to theoretical timelines axis, where temporal relations can only occur within the same axis, spanning; \emph{main} for actual events that have occurred (in past/present time), intentional for events that did not happened but however are intended to happen and hypothetical for events that might happened. (2) Consider only 4 types of temporal relations; \emph{before}, \emph{after}, \emph{equal}, \emph{vague}. (3) Consider only the beginning time of events when deciding on the temporal relation. Those constrains aided MATRES authors in reducing annotation complexity, use non-expert annotators while achieve a rather high Inter Annotation Agreement (IAA). However, METRES method does not reduce the quadruple  complexity of annotating temporal relations and no tool is provided for this annotation scheme. In this work we adopted the axis method and further extended it to the coreference and causal relations, taking into consideration the unique characters of those relations, especially their transitive closure and temporal constraints to reduce annotation complexity.

%The process of annotating those relations is considered very challenging, to that end, datasets such as CaTeRS \cite{mostafazadeh-etal-2016-caters}, RED \cite{ogorman-etal-2016-richer} and MEVEN-ERE \cite{wang-etal-2022-maven} which feature those relations (coreference, temporal and causal) were annotated using expert annotators. Our goal with the releasing of our annotation tool is to make the annotation of such event-knowledge graph resources accessible to non-expert annotators as well. 



==> backup/background_v2.tex <==
\section{Background and Related Work}
\label{sec:background}
This section surveys relevant research on event relation graphs, covering their structure and desired properties (§\ref{back:compl-consist-complex}), datasets restrictions (\S\ref{back:datasets}), and annotation tools (\S\ref{back:annot-tools}).


\subsection{Event Relation Graph} 
\label{back:compl-consist-complex}

An event relation graph consists of nodes, which represent event \textbf{coreference} clusters — groups of event mentions referring to the same real-world event \cite{raghunathan-etal-2010-multi}, and edges, which represent the relations between these clusters. These include \textbf{Temporal} \cite{do-etal-2012-joint} relations, which encode the sequence of events over time, and \textbf{Causal} \cite{chaturvedi-etal-2017-story} relations, which indicate how one event influences another.\footnote{An additional relation type often considered is the sub-event relation \cite{glavas-etal-2014-hieve}, but it is beyond the scope of this work.} 

Notably, understanding temporal, coreference, and causal relations necessitates anchoring events to specific points or intervals on a timeline \cite{caselli-vossen-2017-event, ning-etal-2018-multi}. Temporal relations connect \textit{any} two event mentions and must maintain transitive consistency; that is, if A is before B and B is before C, then A must also be before C. Causal relations link pairs of events where one event \textit{precedes} and causes the other. Coreferring event mentions, referring to the same real-world event, must also \textit{co-occur}.

A valid event relation graph requires linking all event pairs while ensuring transitive consistency \cite{marc-et-al-2005-temporal}. However, annotating every relation in articles of non-trivial length is considered infeasible \cite{naik-etal-2019-tddiscourse}, and inconsistencies among human annotators are frequently observed, as highlighted in the TimeBank corpus \cite{pustejovsky-stubbs-2011-increasing}. Therefore, the primary objective of \App{} is to assist annotators in generating a \textit{complete} and \textit{consistent} event relation graph for a given set of event mentions within a text.


% Notably, understanding temporal, coreference, and causal relations requires anchoring events to specific points or intervals on a timeline \cite{caselli-vossen-2017-event, ning-etal-2018-multi}. Temporal relations connect \textit{any} two event mentions, while causal relations link causally related pairs where one event \textit{precedes} and causes the other. Coreferring event mentions, as they refer to the same real-world event, must also \textit{co-occur}.

%Creating an event relation graph requires the \textit{completeness} and \textit{consistency} of annotations \cite{marc-et-al-2005-temporal}, linking all event pairs without contradictions. However, annotating every temporal relation in an article is considered infeasible \cite{naik-etal-2019-tddiscourse}, and inconsistent annotations are common among human annotators, as seen in the TimeBank corpus \cite{pustejovsky-stubbs-2011-increasing}. Therefore, a primary goal of \App{} is to help annotators produce a consistent and complete event relation graph.

% Creating an event relation graph requires linking all event pairs (\textit{complete}) while ensuring that the annotations are free of contradictions (\textit{consist}) \cite{marc-et-al-2005-temporal}. However, annotating every relation in articles of non-trivial length is consider infeasible \cite{naik-etal-2019-tddiscourse}, and inconsistencies among human annotators are frequently observed, as highlighted in the TimeBank corpus \cite{pustejovsky-stubbs-2011-increasing}. Therefore, the primary objective of \App{} is to assist annotators in generating a \textit{consistent} and \textit{complete} event relation graph for a given set of event mentions within a text.

% \subsection{Annotation Schemes}
% \label{back:annot-schemes}
% Prominent prior works \cite{ogorman-etal-2016-richer, caselli-vossen-2017-event} have adopted the TimeML \cite{pustejovsky2003timeml} annotation scheme to annotate relations between \textit{all} temporal expressions (e.g., dates and times) and events. However, due to its quadratic complexity, using this scheme results in sparsely annotated datasets. 
% Moreover, TimeML does not address cases where relations cannot be determined from the context (i.e., `vague' cases), which can potentially lower inter-annotator agreement as annotators are required to choose a temporal class for the relation (e.g., `after', `before', `equals', etc.).
% %Moreover, TimeML does not account for cases where relations cannot be determined from the context (i.e., `vague' cases), potentially lowering inter-annotator agreement as annotators are required to select a temporal class of the relation (i.e., after, before, equals, etc..). 
% Causal relations annotation, typically follows the RED protocol \cite{ogorman-etal-2016-richer}, which requires evaluating all event pairs, significantly increasing complexity.
% To annotate relations only between temporally anchorable events and streamline causal relation annotation, we adopt the Multi-Axis annotation scheme \cite{ning-etal-2018-multi} for temporal relations and the EventStoryLine methodology \cite{caselli-vossen-2017-event}\footnote{We focus exclusively on the causation relation (excluding enablement and prevention), similar to \citet{ning-etal-2018-joint, do-etal-2011-minimally}.} for causal relations, further detailed in §\ref{tool:annot-schemes}.


\subsection{Annotation Restrictions}
\label{back:datasets}

% To make manual annotation feasible, prior works on event-event relations have restricted the annotation scope. These restrictions are categorized as: 1) systematic reductions, which limit annotation to events in consecutive sentences \cite{chambers-etal-2014-dense, minard-etal-2016-meantime, caselli-vossen-2017-event, ning-etal-2018-joint}, simplifying the process but missing document-wide relations and limiting models' ability to learn long-range dependencies; and 2) non-systematic reductions, which produce incomplete annotations without clear justification \cite{mirza-etal-2014-annotating, ogorman-etal-2016-richer, wang-etal-2022-maven}, potentially introducing undetectable biases.

% To make manual annotation feasible, prior works on event-event relations have limited the annotation scope. These restrictions can be categorized as systematic reductions, with most prior work adopting the approach of focusing on relations between events within consecutive sentences \cite{chambers-etal-2014-dense, minard-etal-2016-meantime, caselli-vossen-2017-event, ning-etal-2018-joint}. This approach simplifies the process but fails to capture document-wide relations. Another common systematic restriction involves concentrating temporal annotations on "narrative containers" \cite{styler-iv-etal-2014-temporal, pustejovsky-stubbs-2011-increasing} — grouping events that can be anchored by dates or temporal expressions and creating temporal relations between them. While these methods organize events around explicit anchors, they might overlook relations that can be inferred using common-sense reasoning.

% To facilitate manual annotation, prior works on event-event relations often constrain the scope by focusing on relations within consecutive sentences \cite{chambers-etal-2014-dense, minard-etal-2016-meantime, caselli-vossen-2017-event, ning-etal-2018-joint} or using ``narrative containers'' \cite{pustejovsky-stubbs-2011-increasing, styler-iv-etal-2014-temporal, ogorman-etal-2016-richer, wang-etal-2022-maven} to group events by temporal anchors. While these approaches simplify annotation and organize events effectively, they fail to capture document-wide relations or those requiring common-sense reasoning.


To facilitate manual annotation, prior works on event-event relations often constrain the scope by focusing on relations within consecutive sentences \cite{chambers-etal-2014-dense, minard-etal-2016-meantime, caselli-vossen-2017-event, ning-etal-2018-joint}. While this simplifies the process, it fails to capture document-wide relations. Another common constraint focuses temporal annotations on ``narrative containers'' \cite{pustejovsky-stubbs-2011-increasing, styler-iv-etal-2014-temporal, ogorman-etal-2016-richer, wang-etal-2022-maven}, which group events anchored by dates or temporal expressions to establish temporal relations. Although this method effectively organizes events around explicit anchors, it may overlook relations requiring common-sense reasoning.

Other constraints are less systematic, such as using automatic tools to assist with annotation \cite{mirza-etal-2014-annotating, madaan-yang-2021-neural, tan-etal-2024-set} or conducting full manual annotations \cite{pustejovsky-etal-2003}. Both approaches, however, often result in sparse datasets without explicit justification and risk introducing biases from either the annotators or the tools employed.

Our objective in developing \App{} is to facilitate dataset creation by constraining the set of events for annotation while ensuring all relations among these events are annotated. Although this approach is limited by event selection, we argue that it has minimal impact on the learning process for event-event relation extraction, as event mentions are provided to the model as input.

% Our objective in developing \App{} is to facilitate the creation of datasets that, rather than limiting the relations set across all events, constrain the set of events considered for annotation while ensuring that all relations among these events are annotated. The primary limitation of our approach lies in the event selection process. However, we argue that this restriction is less likely to influence the learning process within the scope of event-event relation extraction, as event extraction itself is not the focus of this task, given that event mentions are provided to the model as part of the input.

% Our goal in developing \App{} is to support the creation of resources consisting of \textit{complete} relation annotations between all event mentions within a selected subset of events. 


%%%%%%%%%%%%%%%%%%% START PREVIOUS VERSION %%%%%%%%%%%%%%%%%%%
% To annotate causal relations, it is standard practice to follow the RED annotation guidelines \cite{ogorman-etal-2016-richer}, which require assessing all pairs of events, adding significant complexity. To simplify this process, we adopt the EventStoryLine methodology \cite{caselli-vossen-2017-event},\footnote{We only focus on the causation relation (excluding enablement and prevention), similar to \citet{ning-etal-2018-joint, do-etal-2011-minimally}.} which differs from RED by presenting an event alongside \emph{all} its preceding events, requiring annotators to select all the causing event(s) out of these candidates. Our experiments with both methods (Appendix~\ref{app:cause-scheme-expr}) show that the EventStoryLine method is more efficient and achieves higher agreement among annotators than the RED methodology. 
%%%%%%%%%%%%%%%%%%%%%% END PREVIOUS VERSION %%%%%%%%%%%%%%%%%%


% is essential for understanding how one event influences another in a story or narrative \cite{chaturvedi-etal-2017-story}. Unlike a temporal relation, a causal relation exists only between positively identified pairs; all other pairs are considered negative examples.


% Notably, causal relations are also directly governed by temporal relations; naturally, an event that causes another must precede it.


%Since our approach aims to reduce the quadratic annotation complexity necessary for achieving a complete event relation graph.  In contrast to RED, this methodology presents each tail event alongside \emph{all} preceding events. Annotators are tasked with determining \emph{why the tail event occurred} and identifying if the cause is among the listed candidates (head events). Our experiments (detailed in §\ref{app:cause-scheme-expr}) demonstrate that this method is more efficient and achieves higher agreement among annotators then the RED methodology. Notably, causal relations are also directly governed by temporal relations; naturally, an event that causes another must precede it.

%In contrast, the EventStoryLine methodology \cite{caselli-vossen-2017-event} presents each tail event alongside all preceding events. Annotators are tasked with determining \emph{why the tail event occurred} and identifying if the cause is among the listed candidates. Our experiments (detailed in §\ref{tool:logic}) demonstrate that this method is more efficient and achieves higher agreement among annotators. Therefore, we have adopted the EventStoryLine approach in \App{}.\footnote{We only consider the causal relation (without enablement), similar to \citet{ning-etal-2018-joint, do-etal-2011-minimally}.}

%For the causal annotation, we adopt the annotation methodology from EventStoryLine \cite{caselli-vossen-2017-event},\footnote{We only consider the causal relation (without enablement), similar to \citet{ning-etal-2018-joint, do-etal-2011-minimally}.} where each tail event is presented with all preceding events. The annotator needs to determine \emph{why the tail event has happened} and then verify if the causing event is among the listed candidates. This in contrast to the RED \cite{ogorman-etal-2016-richer} annotation methodology, where given an event pair, involves assessing if \emph{the tail event is inevitable given the head event}. We further discuses our motivation for adopting the EventStoryLine methodology in §\ref{tool:logic}.

%The coreference and causal relations are constrained by the temporal relation. Event mentions that corefer must be identical in time and duration. For an event to cause another, it must start \emph{before} the affected event.


% \subsection{Completeness and Consistency}
% \label{back:compl-consist-complex}


%by identifying all pairs of events that require annotation and preventing contradictions in direct, transitive, and across different types of relations (for example, a \emph{cause} must align with a \emph{before} temporal relation). (2) Reducing annotation \emph{complexity} to make the process feasible and manageable for annotators.

% To that end \App{} is integrated with a framework that enforce these attributes, as further detailed in §\ref{tool:logic}.

\subsection{Existing Annotation Tools}
\label{back:annot-tools}

%Existing datasets that encompass the temporal, coreference and causal relations (or a subset of these relations) \cite{chaturvedi-etal-2017-story, mirza-etal-2014-annotating, hong-etal-2016-building, ogorman-etal-2016-richer, wang-etal-2022-maven}, have either utilized and customized general-purpose tools such as BRAT \cite{stenetorp-etal-2012-brat} or CAT \cite{bartalesi-lenzi-etal-2012-cat}, or did not release or specify the use of any annotation tool.

%Currently, to establish multiple event-event relation annotation, two options are available: (1) using general-purpose annotation tools like BRAT \cite{stenetorp-etal-2012-brat} and CAT \cite{bartalesi-lenzi-etal-2012-cat}, which offer extensive customization and administrative capabilities. 
%However, they lack specific implementations crucial for managing the complexity of event relation annotations by ensuring completeness and consistency. (2) using multiple event annotation tools, each dedicated to a specific relation type. Yet, all temporal annotation tools \cite{cassidy-etal-2014-annotation, derczynski-etal-2016-gate, fulda-etal-2016, rogers2022narrativetime} follow the TimeML annotation scheme, while no existing tool that we know of supports causal annotation. Furthermore, using multiple tools to annotate different types of relations presents significant challenges in terms of management and maintenance. To address these issues, we developed \App{} to meet specific needs of event relation annotation within a single unified workflow.

% Currently, There are two primary methods for annotating multiple event-event relations. One method involves adapting \textit{general-purpose} annotation tools like BRAT \cite{stenetorp-etal-2012-brat} and CAT \cite{bartalesi-lenzi-etal-2012-cat} for constructing relation graphs. 
% However, these tools lack specific features for addressing the specific needs of event relation annotations, such as ensuring completeness, consistency, and leveraging the characteristics of such graphs to manage complexity. 
% The other method involves using multiple dedicated tools, each for a specific type of relation. 
% Yet, existing annotation tools for temoral relations \cite{cassidy-etal-2014-annotation, derczynski-etal-2016-gate, fulda-etal-2016, rogers2022narrativetime} adhere to the TimeML annotation scheme, and none support causal relations annotation.
% Additionally, using multiple tools poses challenges in terms of management and maintenance. 
% To address these issues, we develop \App{}, designed specifically for annotating multiple event-event relations within a unified workflow.

Currently, there are two primary methods for annotating multiple event-event relations. The first involves adapting \textit{general-purpose} annotation tools, such as BRAT \cite{stenetorp-etal-2012-brat} and CAT \cite{bartalesi-lenzi-etal-2012-cat}. However, these tools lack features specifically designed for event relation annotation, such as ensuring completeness, consistency, and managing annotation complexity. The second method employs multiple dedicated tools for specific types of relations. Yet, existing tools for temporal relations \cite{cassidy-etal-2014-annotation, derczynski-etal-2016-gate, fulda-etal-2016, rogers2022narrativetime} adhere to systematic annotation schemes \cite{pustejovsky2003timeml}, and no annotation tool supports causal relation annotation. Additionally, the use of multiple tools introduces further challenges. We developed \App{} to address this gap and enable the annotation of multiple event-event relations within a single unified workflow.


%%%%%%%%%%%%%%%%%%% START PREVIOUS VERSION %%%%%%%%%%%%%%%%%%%
% Currently, there are two main approaches to annotating multiple event-event relations: (1) using general-purpose annotation tools like BRAT \cite{stenetorp-etal-2012-brat} and CAT \cite{bartalesi-lenzi-etal-2012-cat}, adapted for relation graphs. However, these tools lack specific features crucial for managing the complexity of event relation annotations, such as ensuring completeness, consistency, and effectively handling complexity. (2) employing multiple dedicated tools, each for a specific type of relation. Yet, all known temporal annotation tools \cite{cassidy-etal-2014-annotation, derczynski-etal-2016-gate, fulda-etal-2016, rogers2022narrativetime} adhere to the less-efficient TimeML annotation scheme, and there are no existing tools that support causal annotation to our knowledge. Furthermore, using multiple tools poses significant challenges in terms of management and maintenance. In response to this gap, we developed \App{} to specifically cater to the needs of multiple event-event relations annotation within a single unified workflow.
%%%%%%%%%%%%%%%%%%%% END PREVIOUS VERSION %%%%%%%%%%%%%%%%%%%%%%


% To the best of our knowledge, \App{} is the first annotation tool to support end-to-end annotation of temporal, causal, and coreference relations, enforcing completeness and consistency while managing complexity (further detailed in §\ref{tool}).

% In the individual relation annotation space, a variety of tools have been developed over the years for specific tasks, such as temporal relation annotation \cite{verhagen-etal-2006-annotation, verhagen-pustejovsky-2008-temporal, cassidy-etal-2014-annotation, derczynski-etal-2016-gate, fulda-etal-2016, rogers2022narrativetime}, and coreference \cite{girardi-etal-2014-cromer, oberle-2018-sacr, bornstein-etal-2020-corefi}.\footnote{To the best of our knowledge, no tool exists specifically for annotating causal relations.} However, most temporal annotation tools adhere to the TimeML scheme. Additionally, using multiple tools to annotate different types of relations poses significant challenges in terms of handling and maintenance.



==> backup/intro_text.tex <==
% The main types considered for relations that might hold between events, are: \textbf{Temporal} \cite{do-etal-2012-joint}, \textbf{Causal} \cite{chaturvedi-etal-2017-story}, and \textbf{Coreference} \cite{raghunathan-etal-2010-multi}.

% Despite the importance of the task, high-quality and densely annotated resources are rather scarce. 
% \avivs{I would write a short paragraph talking about why the task is important, for motivation, and then I would open a new paragraph starting with this sentence ("despite its importance, resources are scarce.") and discussing the potential reasons.}

% Despite their importance, densely annotated event relation graphs are rare and most prior work, including \cite[RED;][]{ogorman-etal-2016-richer}, \cite[EER;][]{hong-etal-2016-building}, and \cite[MAVEN-ERE;][]{wang-etal-2022-maven}

% due to the challenging annotation and the quadratic complexity involved in annotating such graphs \cite{rogers2022narrativetime}. 
% Existing annotation tools typically focus on general graph annotation \cite{stenetorp-etal-2012-brat, bartalesi-lenzi-etal-2012-cat} and do not effectively address the specific needs of event-relation graphs, often requiring separate annotations for each relation type. 
% Few tools that target event relations only focus on either temporal relations \cite{fulda-etal-2016, rogers2022narrativetime} or coreference \cite{oberle-2018-sacr, bornstein-etal-2020-corefi}.

% Despite their importance, high-quality, densely annotated event relation graphs are rare due to the challenging annotation and the quadratic complexity involved in annotating complete relation graphs \cite{rogers2022narrativetime}.
% Existing annotation tools typically focus on general graph annotation \cite{stenetorp-etal-2012-brat, bartalesi-lenzi-etal-2012-cat} and do not effectively address the specific needs of event-relation graphs, often requiring separate annotations for each relation type. 
% Few tools that target event relations only focus on either temporal relations \cite{fulda-etal-2016, rogers2022narrativetime} or coreference \cite{oberle-2018-sacr, bornstein-etal-2020-corefi}.

% This scarcity may stem from the complex nature of annotating event relations, which can be challenging even for experts, with several prominent datasets reporting low low Inter-Annotator Agreement (IAA) \cite{hong-etal-2016-building, ogorman-etal-2016-richer, styler-iv-etal-2014-temporal}.
% Additionally, the quadratic complexity involved in annotating complete relation graphs further complicates the creation of \textit{densely} annotated datasets \cite{rogers2022narrativetime}. As a result, most datasets are not dense in nature, and those that do try to achieve higher density, mainly focus on events in consecutive sentences \cite{cassidy-etal-2014-annotation}.

% Existing datasets and tools mainly address temporal relations derived from explicit temporal expressions like `before' or `while', neglecting implicit event connections. 
% This scarcity may stem from the complex nature of annotating event relations, which can be challenging even for experts. 
% Indeed, this complexity is reflected in the low Inter-Annotator Agreement (IAA) scores of common datasets, such as below 20\% for the Event-Event Relation dataset \cite{hong-etal-2016-building} and below 60\% for the Richer Event Description \cite[RED;][]{ogorman-etal-2016-richer} and THYME-TimeML \cite{styler-iv-etal-2014-temporal} datasets. 
% Additionally, the quadratic complexity involved in annotating complete relation graphs further complicates the creation of \textit{densely} annotated datasets \cite{rogers2022narrativetime}. As a result, most datasets are not dense in nature, and those that do try to achieve higher density, mainly focus on events in consecutive sentences \cite{cassidy-etal-2014-annotation}.

% However, high-quality, densely annotated event relation graphs are scarce, and none are exhaustively annotated. In fact, most datasets and annotation tools primarily focus on temporal relations, specifically temporal relations that are entailed from temporal expressions such as `before' or `while', thereby neglecting event mentions that are linked implicitly. 
% This scarcity may stem from the challenging nature of the annotation process, since identifying specific relations between events is a complex linguistic task, even for expert annotators.
% For example, the average Inter-Annotator Agreement (IAA) in the Event-Event Relation dataset \cite{hong-etal-2016-building} was below 20\%, and in the Richer Event Description \cite[RED;][]{ogorman-etal-2016-richer} and THYME-TimeML \cite{styler-iv-etal-2014-temporal} datasets, it was below 60\%, demonstrating the complexity of the task.
% Additionally, annotating complete relation graphs is quadratically complex, requiring evaluation of relations between \textit{all} event pairs. Consequently, most existing datasets lack densely annotated event relations, usually focusing only on events in consecutive sentences \cite{rogers2022narrativetime}.


%Following the Multi-Axis annotation scheme \cite{ning-etal-2018-multi}, \App{} first identifies event mentions anchored in time,\footnote{Events that have already happened or will happen.} and then annotates all three relation types for each pair of these mentions. 
% Specifically, the annotation process iterates through four manageable, self-contained steps--identifying relevant event mentions and separately annotating each of the relation types for each pair of event mentions.
%On an input document with marked event mentions ((1) in Figure~\ref{fig:figure1}), annotators start by identifying the event mentions that are anchored in time (§\ref{tool:event-select}). 
%Next, they proceed to annotate temporal relations between all pairs of anchored event mentions (§\ref{tool:temp}), deciding which event occurred first ((2) in Figure~\ref{fig:figure1}).
%To reduce workload, \App{} uses a transitive closure algorithm to infer and auto-annotate unattended pairs from existing annotations, while also ensuring consistency by detecting and alerting annotators to any contradicting relations.

%After temporal annotations, \App{} proceeds to coreference annotation (§\ref{tool:coref}). Annotators are given an event mention and a list of event mentions and must select the coreferring ones ((3) in Figure~\ref{fig:figure1}). By leveraging temporal annotations from the previous step to focus only on co-occurring event pairs, we reduce the workload by 95\% \cite{ogorman-etal-2016-richer, rogers2022narrativetime}.

% Upon completing the temporal relation annotation, \App{} proceeded to the coreference annotation step (§\ref{tool:coref}). Here, annotators are presented with an event mention and a list of potentially coreferring event mentions, and are tasked with choosing which corefer to the event in question ((3) in Figure~\ref{fig:figure1}). Notably, we leverage the temporal annotations from the previous step to only focus on event mention pairs which were labeled as co-occuring, thereby reducing the total workload by 95\%  \cite{ogorman-etal-2016-richer, wang-etal-2022-maven, rogers2022narrativetime}.

%The final step involves annotating causal relations (§\ref{tool:cause}). Annotators are presented with an event mention and a list of preceding events, derived from step (2), and they must select which events caused the given event ((4) in Figure~\ref{fig:figure1}). This approach follows the EventStoryLine method  \cite{caselli-vossen-2017-event}, which we have found to be more intuitive and yield higher agreement among annotators than other annotation approaches. Additionally, we use coreference annotations from the previous step to group coreferring mentions into a single event, further reducing workload.




% identifying relevant event mentions (§\ref{tool:event-select}), and separately annotating temporal (§\ref{tool:temp}), coreference (§\ref{tool:coref}), and causal (§\ref{tool:cause}) relations for each pair of event mentions.




% \App{} simplifies the annotation process by decomposing it into four manageable, self-contained steps (shown in Figure~\ref{fig:figure1}): identifying relevant event mentions (§\ref{tool:event-select}), and separately annotating temporal (§\ref{tool:temp}), coreference (§\ref{tool:coref}), and causal (§\ref{tool:cause}) relations for each pair of event mentions.
% This approach ensures comprehensive coverage, including events not linked by explicit temporal expressions, thus promoting dense annotations.
% By leveraging transitive relations, as well as the connections between the different relation types, \App{} significantly reduces the overall annotation workload, cutting down the number of pairs requiring \textit{manual} annotation by over 60\% for temporal relations and by 95\% for coreference relations (§\ref{tool}).
% We also ensure consistent and exhaustive annotations by checking for contradictory or missing relations and alerting annotators as needed.


% To simplify the annotation process, we decompose it into four manageable, self-contained steps (shown in Figure~\ref{fig:figure1}): identifying relevant event mentions (§\ref{tool:event-select}), and separately annotating temporal (§\ref{tool:temp}), coreference (§\ref{tool:coref}), and causal (§\ref{tool:cause}) relations for each pair of event mentions. By inspecting each pair, our annotation process manages to also address event mentions that are not necessarily linked via a temporal expression, making this process more exhaustive than the previous approaches.
% We leverage transitive relations and the connections between the different relation types to reduce the overall annotation workload, cutting the number of event pairs requiring manual annotation by over 60\% for the temporal relations, and by 95\% for the coreference relations (§\ref{tool}).
% Additionally, we ensure high-quality annotations by checking for contradictory or missing relations and alerting annotators as needed.

% The results of our study indicate that our tool significantly simplifies the annotation process, while also enabling high-quality annotations, as indicated by the enhanced Inter-Annotator Agreement (IAA).
% Overall, \App{} combines different techniques and practices for streamlining the complex annotation process of event relations, while also adding safeguards to ensure consistency and completeness, thereby enabling a \textit{single} intuitive framework for annotating temporal, coreference, and causal relations. 
% The tool and code are publicly available at \url{https://github.com/AlonEirew/EventGraphAnnot}.



% To address these limitations, there is a need for an annotation tool that can facilitate the complex task of annotating an exhaustive event-event relation dataset among all events in the text. However, to the best of our knowledge, no such tool is publicly available (see §\ref{back:annot-tools}).
% \avivs{This entire paragraph should be rephrased as "To address these limitations, we develop..." (basically the following paragraph). Omit the whole "there is a need..." and "no such tool is publicly available". The latter can be said implicitly as "To address these limitations, we present \App{}, a *novel* annotation tool..."}


% To that end, we developed a tool designed to assist in the complex task of exhaustively annotating event-event relations, covering temporal, coreference, and causal types. We simplify the annotation task by breaking it down into smaller, manageable, and self-contained steps (illustrated in Figure~\ref{fig:figure1}). we experiment and integrated annotation methodologies that provide simplicity and high agreement between annotators (§\ref{tool:annot-flow}). 

% Additionally, our tool provides an algorithmic framework (§\ref{tool:logic}) that reduce the annotation complexity (the number of annotation steps required) by up to 60\%, enforce consistency (avoid contradicting relations), and completeness (ensure all relations are covered) of annotation, in the aim of producing high quality resources.

% To evaluate the effectiveness of our tool, we conducted a pilot study (§\ref{pilot}). The results of our study indicate that our tool simplifies the annotation process and enhances Inter-Annotator Agreement (IAA) among annotators.

% \avivs{contributions: (1) environment to annotate all relation together (2) it enables do it dense (exhaustive of all pairs) on any manageable size of events without any constraints where they appear i.e. can appear anywhere in the document and not only e.g. in consecutive sentences, which is complex because of quadratic quantity. (3) efficiency - transitivity/coref only on coinciding/task order/causal only on events coming after (4) discrepancy-checking (has been done in some previous works) --> and all this wrapped up in a single tool.}
% \avivs{Make sure there are enough examples of printscreens.}
% \alone{There is another small contribution that might be worth mentioning: the tool can be customized to support the annotation of a subset of relations (e.g., temporal and causal) or only temporal relations in isolation. I'm not sure where (or if) to add this.}




%% OLDER DATA BELOW
% \avivs{Is this information relevant? maybe say generally that there are different types of relations, listing them only by name (and reference), and then further explain about each on in the following sections?}

%Meanwhile, the identification and extraction of event-event relations continue to pose significant challenges to contemporary generative Large Language Models \cite{gao-etal-2023-chatgpt, peng2023does}.

%whether in isolation or as part of a more comprehensive knowledge graph is beneficial in many downstream tasks such as information consolidation \cite{hirsch-etal-2021-ifacetsum}, information retrieval \cite{eirew-etal-2022-cross}, and is being applied in several domains such as medical \cite{Li2020TimeEO}, legal and others. Yet,
%this research filed continue to pose significant challenges to contemporary generative Large Language Models (LLMs) \cite{gao-etal-2023-chatgpt, peng2023does}.

%In this research we focus on the first three relations (temporal, coreference and causal), which considered the most studied event relation extraction (ERE) task relations.

%The availability of resources for extracting the above event-event relations jointly, remains notably limited. To the best of our knowledge, Event-Event Relation (EER) \cite{hong-etal-2016-building}, Richer Event Description (RED) \cite{ogorman-etal-2016-richer}, EventStoryLine (ESL) \cite{caselli-vossen-2017-event}, and MAVEN-ERE \cite{wang-etal-2022-maven} are the only datasets currently available that encompass all three relations. 

%Additionally, all prior related work—including RED, EventStoryLine \cite{caselli-vossen-2017-event}, and MAVEN-ERE \cite{wang-etal-2022-maven}, were annotated following the TimeML \cite{pustejovsky2003timeml} annotation scheme. This scheme necessitate the anchoring of events to explicity time expressions.
%or the document creation time (DCT). 
%This approach alleviate both challenges of disagreement and annotation complexity. However, it generates sparse temporal annotations between events, which subsequently impact the density of causal and coreference relations, as those are temporally constrained (further discussed in §\ref{tool:annot-flow}). 

%Furthermore, while temporal relations inherently exist between any pair of events, allowing us to disregard unjudged event pairs when training or testing a model, causal and coreference relations might not exist between events. Thus, incompletely annotated causal and coreference relations might cause unjudged pairs to mistakenly be considered as negative examples.

%Second, the time anchoring constraint might overlook event-event relations that can be inferred using common-sense reasoning and world knowledge. For example, it is commonly understood that dessert is served after the main course or that someone must be kidnapped before a ransom is demanded. As a result, this method partially removes the challenge of applying common-sense reasoning.

%We employ the novel Multi-Axis temporal event-event annotation scheme \cite{ning-etal-2018-multi} (discussed further in §\ref{back:multi}) to ground temporal relations between events. 
%that share similar semantic properties (actual vs. non-actual). 

%To tackle the challenges of annotation complexity, consistency, and completeness, we have developed an algorithmic framework (discussed further in §\ref{tool:logic}). This framework automatically fills in transitive relations, alerts annotators on potential contradictions that need fixing, and ensures that no relation is overlooked.

%Second, to address the challenges of annotating such a resource, we experiment and integrated annotation methodologies that provide simplicity and high agreement between annotators (§\ref{tool:annot-flow}). Additionally, our tool provides an algorithmic framework (§\ref{tool:logic}) that address the complexity (the number of annotation steps required), consistency (avoiding contradicting relations), and completeness (ensuring all relations are covered) of annotation, in the aim of producing high quality resources. 

%that: (1) automatically fills in inferred relations based on previous annotations, thus reducing the number of annotation steps required; (2) ensures annotation completeness to guarantee that no relation is overlooked, and maintains consistency by alerting annotators to potential contradictions that need resolution. 

%Creating an ERE resource that is exhaustively annotated between events is a very challenging task. Besides the linguistic challenge and the quadruple annotation complexity, we aim to create a graph that is complete and consistent. This consideration is often overlooked when building a new resource for the task \cite{pustejovsky-stubbs-2011-increasing}. However, ensuring consistency can be challenging for annotators, given the many relations that need to be considered and the necessity of keeping track of all transitive relations.

%This lack of resources can be largely attributed to the challenging annotation process. First, identifying the specific relation between two events is considered a difficult linguistic challenge. For instance, the average Inter-Annotator Agreement (IAA) in EER was below 20\% and in RED was below or near 60\%. Second, annotation complexity arises when considering a set of events, as annotators are required to assess the relation between each pair of events, resulting in a quadratic complexity for each individual relation type. To that end, none of the previous works performed exhaustive annotation between events (this is further discussed in §\alone{add to background}). However, incomplete graphs can hinder the training process, as models might generate a correct relation but get penalized as it is missing from the training set.

%Another important aspect that requires attention when annotating ERE datasets is ensuring consistency to minimize the number of contradictory relations that might surface. This consideration is often overlooked when building a new resource for the task \cite{pustejovsky-stubbs-2011-increasing}. However, ensuring consistency can be very challenging for annotators, given the many relations that need to be considered and the necessity of keeping track of all inferred relations. 

%Among the relations, the most challenging and perhaps the most important is the temporal relation. This importance is derived from the fact that both coreference and causal relations are constrained by the temporal relation between events (equal for coreference, and before/after for cause/effect). Additionally, temporal relations are challenging because not all temporal relations can be inferred from the text, as writers often focus on advancing their story in an engaging way rather than spelling out all the details \cite{rogers2022narrativetime}.

%EventStoryLine, RED, and MAVEN-ERE all adopted the TimeML \cite{pustejovsky2003timeml} annotation scheme. This scheme anchors events to time expressions and the document creation time (DCT), alleviating to some degree the disagreement challenge. However, this time anchoring constraint skips event-event relations that can be inferred using common-sense reasoning. For example, we can understand that dessert comes after the first course or that someone needs to be kidnapped before a ransom is demanded, without explicitly relying on time expressions. This approach creates a rather sparse annotation density between events \cite{chambers-etal-2014-dense, reimers-etal-2016-temporal, ning-etal-2018-multi}.

%Additionally, to alleviate the quadruple complexity of relation annotation, other works annotate only relations that span across adjacent sentences \cite{chambers-etal-2014-dense, minard-etal-2016-meantime} \alone{add TCR}, select short documents for the task \alone{Add CaTeRs}, or only annotate part of the document \cite{caselli-vossen-2017-event}.

%However, MAVEN-ERE, derived primarily from the leading section of Wikipedia articles, presents specific challenges due to its domain-centric nature. Meanwhile, RED is characterized by relatively sparse annotations \alone{Cite paper saying this}. This resource scarcity highlights the need for additional datasets for this challenging task.

%Identifying and extracting event-event relations, if in isolation or as a knowledge graph, is still considered and important and challenging task to modern LLM's \cite{gao-etal-2023-chatgpt, peng2023does} and a benchmark for models knowledge \cite{yu2023kola}. Yet, the availability of resources for extracting event-event knowledge graphs remains notably sparse. 

%Other efforts have been made to generate datasets with a smaller set of relations, such as single-relation datasets \alone{cite single datasets}, and datasets containing pairs of relations \alone{cite related work}. However, those resources are all sparsely annotated between event mentions, and we found that some of them contain contradictory relations.

%Last, when creating a resource for this task, it is important to ensure that relations do not contradict each other, whether in transitive relations or by other relation types that impose constraints between relations.

% For instance, during the annotation of MAVEN-ERE \cite{wang-etal-2022-maven}, dozens of annotators were employed to manage its scale. Other related works have taken a more limited approach to scale down the annotation complexity, by only considering a sub-set of all events or restricting their annotations to only consider events from adjacent sentences \cite{chambers-etal-2014-dense, ning-etal-2018-multi}.

%Some studies, have developed their own annotation tools \cite{hong-etal-2016-building} or have conducted annotations without indicating the use of any specific tool \cite{wang-etal-2022-maven}.

%The benefits of using general purpose tools such as Brat and CAT for the event-event relation annotation is rather limited. While they provide rich customization, visual and administrative aid (calculating IAA, tracking annotator progress, etc.), since they are not designed for event-event relation annotation, customization is ad-hoc and cannot be used by future developer of such resouces. Visualization can become rather dense and unhelpful when annotating many events. They do not consider the special characteristics of event-event relation (such as transitive closure) or the temporal constrains of causal and coreference relations to provide reduction in the annotation complexity.

%To address these challenges we present in this work a comprehensive tool to create an exhaustive ERE dataset that enforces annotation completeness and consistency, while significantly reducing the complexity of the annotation process.

%To achieve this, we break down the comprehensive and complex annotation task into smaller, manageable, and self-contained steps (illustrated in Figure~\ref{fig:figure1}). We utilize the Multi-Axis \cite{ning-etal-2018-multi} annotation scheme (further discussed in §\ref{back:coref-cause-temp}) for grounding events and simplifying the annotation of temporal relations. To address the annotation complexity, we introduce two methods: 1) limiting the annotation of coreference and causal relations by their temporal constraints, and 2) developing an algorithmic framework (further discussed in §\ref{tool:logic}) specifically designed to address the unique and spatial characteristics of each event relation. This framework operates in the background during the annotation process, removing the need to annotate transitively inferred relations while performing both completeness and consistency checks. 

%Lastly, we provide the annotators with visual aids and clear instructions (further discussed in §\ref{method:feat}). Using our tool, annotators achieved \alone{Need to add here some statistics after we do the system experiments} IAA, which is considered rather high for this task and on average annotators were required to do significantly less annotation steps \alone{reference to a table that present annotation statistics for each relation}.


%\begin{enumerate}[label=(\alph*)]
%    \item Simplify the annotation process by breaking it into smaller steps (\alone{cite paper that discuss layered annotation}), making it accessible to non-expert annotators.
%   \item Taking advantage of previous annotation schemes (\alone{cite METRES and MAVEN-ERE}) to further simplifying the annotation process and increasing IAA.
%  \item Use existing and develop novel algorithms that significantly reducing annotation complexity to promote exhaustive event-event relation annotation. %This by considering the natural ordering of events in text, the temporal constraints of the causal and coreference relation and the unique transitivity nature of each relation while annotation is performed.
%    \item Speedup the annotation process by suggesting pairs to annotate only considering pairs that thier relation cannot be deduced. 
%    \item Increase IAA with discrepancies check while annotation is preformed.
%    \item Provide a visual aid that present only relevant relations for a specific annotation step.
%    \item Preserve a high degree of customization and flexibility in the annotation scheme of future work that might like to adopt a different annotation scheme. 
%\end{enumerate}


==> backup/pilot_v2.tex <==
\section{Pilot Study}
\label{sec:pilot}

To evaluate \App{}'s effectiveness, we conducted a small-scale study to assess the time and effort required for annotation and the quality of the resulting annotations.
This section details the annotation procedure (§\ref{sec:pilot-annot-proc}) and reviews the quality and effectiveness of the annotation process (§\ref{sec:pilot-analysis}).

%involving three non-expert annotators who received training for each task. This trial 
%We evaluated the annotation we considered two aspects of the annotation: (1) We selected 6 documents from the TCR  dataset. Within each document, 10 gold mentions were chosen according to the following criteria: events participating in causal relationships were given priority 

%from each document we  which the annotators then annotated end-to-end using \App{}. 

\subsection{Annotation Procedure}
\label{sec:pilot-annot-proc}
For the user study, we hired three non-expert annotators, all native English speakers and either first-degree students or graduates. They first underwent 2-3 training iterations on each sub-task using 2-3 test documents to ensure a thorough understanding of the tasks. The actual annotation was conducted on six news documents, each approximately 500 words. To extract the initial set of event mentions, we used the event detection method proposed by \citet{cattan-etal-2021-cross-document}, \alone{which extracted an average of 60 event mentions per document.} Annotators begin by identifying ``anchorable'' event mentions (§\ref{sec:tool-flow}). On average, 35 ``anchorable'' events were identified per document, from which the 16-18 most salient events are selected to manage the study’s scope. After this, annotators proceed to annotate the three event relation types.

For temporal relations, annotators are instructed to first read the article and annotate the most obvious temporal relations by clicking on the relevant edges in the accompanying graph visualization. This approach has proven effective in helping them better understand the underlying story and avoid simple mistakes. 
Since this initial pass usually yields only a few annotations, they then make a second pass to address the remaining pairs.
For coreference and causal relations, annotators are instructed to use the ``Next Unhandled'' button to progress through the annotations.
At any point, annotators can revise annotations as needed using the navigation buttons (available in all steps) or the graph visualization (editable only in the temporal step).
Finally, we measure Inter-Annotator Agreement (IAA), annotation time, and the number of annotation steps for each phase.



% Annotators first identify \textit{anchorable} event mentions (§\ref{tool:event-select}), limited to no more than 18 per document to manage the study’s scope, followed by the annotation of the three event relation types.
% For temporal relations, annotators are instructed to first read the article and annotate clear temporal relations, by clicking on the relevant edges in the accompanying graph visualization. 
% We found that this approach helped them get a better understanding of the underlying story as well as avoid simple mistakes. Upon annotating the entire document once, annotators make a second pass to attend to the unannotated pairs, via the ``Next Unhandled Pair''. 
% For coreference and causal relations, they are instructed to only use the ``Next Unhandled Event'' button for navigation. 
% At any point, annotators can use the navigation buttons to revise earlier annotations as needed.
% Finally, we measure Inter-Annotator Agreement (IAA), annotation time, and number of annotation steps for each step.

%%%%%%%%%%%%%%%%%%% START PREVIOUS VERSION %%%%%%%%%%%%%%%%%%%
% Annotators first identify the \textit{anchorable} event mentions (§\ref{tool:event-select}), limited to no more than 18 mentions per document for the purposes of the user study.
% Next, they proceed with the annotation of the three event relation types. For temporal relations, we instruct them to first read the article carefully, and whenever coming across event mention pairs whose temporal relation is easily understood, to annotate them using the tool's graph visualization feature, by clicking the relevant edge and annotating it.
% We found that this approach helps annotators get a better understanding of the underlying story and later avoid simple errors. Upon completing one pass over the document, they are asked to make a second pass, beginning with the first unannotated pair in the document and following the tool's suggestions via the `Next Unhandled Pair'' button. For coreference and causal annotations, annotators are instructed to use only the Next Unhandled Event'' button for navigation. At any stage, they can modify previous annotations as needed, via the navigation buttons.
% Finally, we measure the Inter-Annotator Agreement (IAA), annotation time, and number of annotation steps for each individual step.
%%%%%%%%%%%%%%%%%%%%%% END PREVIOUS VERSION %%%%%%%%%%%%%%%%%%



%Subsequently, one of the paper's authors reviewed the event mentions in each document and selected 15-18 mentions from each to further reduce annotation scope.
%For the annotation process we selected six news documents, each containing an average of 500 words. As a preliminary step, we used the model from \cite{cattan-etal-2021-cross-document} to extract event candidates from each document. Subsequently, each annotators were given the six document along with \App{} and was tasked with the initial step of assigning events to their correct axis (§\ref{tool:annot-flow} step 1). Following this, one of the authors reviewed the events and selected from each document 13-18 events that are on the main axis and most relevant to the underlying story.


%\cite{fabbri-etal-2019-multi} corpus. The motivation for selecting this resource is that the CNN summaries nicely cover the unfolding of major events and are considered challenging news articles (\alone{find citation for last sent or remove}). We selected summaries that cover at least five articles, each with an average of 500 words per summary.

% For the temporal annotation, we spitted the 15 documents to three groups each with 5 documents. Each group was assign to two different annotators which separately conducted the temporal relation annotation (§\ref{tool:annot-flow} step 2). Following this step we measure the IAA, time and number of annotation steps (presented next in §\ref{pilot:results}) for the temporal relation annotation task.

%For the temporal annotation, we divided the 15 documents into three groups, each consisting of 5 documents. Each group was assigned to two different annotators who independently conducted the temporal relation annotation (§\ref{tool:annot-flow} step 2). We instructed the annotators to first read the entire article without making any annotations. Then, during the second pass, they were to use the graph visualization tool (§\ref{tool:feat}) to annotate pairs between which they had already identified the relation. Finally, we asked the annotators to proceed by using the "Next Unhandled Pair" feature to annotate the remaining pairs.

%Following this step, we measured the Inter-Annotator Agreement (IAA), time, and number of annotation steps for the temporal relation task.

%Next, each group of documents was assigned to the third annotator who had not previously worked on that group. This annotator's role was to adjudicate all relations on which the first two annotators disagreed. This consolidation step is crucial for dense annotation, as subsequent steps are constrained by the temporal relations established here—\emph{equal} for coreference and \emph{before/after} for causal relations (§\ref{tool:annot-flow} step 3). This step ensures that in the next steps, annotators are presented with (1) all relevant temporal relations, and (2) a unified set of candidates.

%After the consolidation step, for the final two steps—coreference and causal relations annotation—all three annotators were given the same five sampled documents to annotate. We then measured the Inter-Annotator Agreement (IAA), time, and number of annotation steps for this task. 
%The results are presented in the following section §\ref{pilot:results} and in Table~\alone{ref to table}.

\input{latex/tables/agree_tab}

\subsection{Analysis}
\label{sec:pilot-analysis}
% \avivs{Should use better discourse, e.g., "We first note that..."} 
\alone{The final annotated set, consisting of 6 documents, included 102 event mentions (an average of 17 mentions per document) and 816 relations (excluding symmetric pairs), with an average of 136 relations per document. In comparison, the MATRES \cite{ning-etal-2018-multi} dataset\footnote{Widely adopted for the temporal relation extraction task.} contains an average of 22 event mentions and 50 relations per document.}

\alone{First, to verify the accuracy of the annotations, one of the authors randomly selected 50 pairs from the documents for blind annotation. The results showed agreement on 46 relations.}

Notably, as shown in Table~\ref{tab:annot_agree}, agreement between annotators is high across all three relations. This indicates that our annotation tool effectively supports the generation of high-quality annotations while maintaining completeness and consistency.
We also observe in Table~\ref{tab:annot_time} that the annotation of temporal relations roughly takes 44.3 minutes to complete, which is significantly more demanding than the other two types of relations. 
%the latter two relations benefit from the temporal relation annotation to further reduce the overall workload.
This finding is sensible, given that temporal relation annotation requires making one of four possible decisions (e.g., before, after, equal, or vague) for each presented pair, and annotators may also need to resolve discrepancies in annotations. In contrast, coreference and causal relations involve identifying connections within a set of events relative to a focal event and its temporal context (\textit{equal} for coreference and \textit{after} for causal). 
Importantly, Table~\ref{tab:annot_step} indicates that \App{} assists in significantly reducing complexity for all three relation types.
\\~\\
Overall, our annotation process generates complete and consistent graphs covering temporal, causal and coreference relations while maintaining simplicity. 
The use of transitive closure algorithms reduced the manual workload for temporal relation annotation by 56\% and prevented inconsistency errors, along with the discrepancy identification algorithm.
Our decision to use the EventStoryLine approach over the RED approach for causal relation annotation, based on preliminary analyses showing higher annotator agreement with the former,\footnote{See Appendix~\ref{app:cause-scheme-expr}.} has also proven effective.
Finally, the task order also helped in streamlining the annotation process. Beginning with temporal relation annotation allowed subsequent steps to focus only on the relevant subset of pairs, leveraging the time constraint between temporal and other relations. This was particularly effective for coreference annotation, where the workload was reduced by 96\% (see Table~\ref{tab:annot_step}). Additionally, annotating coreference before causal relations enabled us to treat coreferring event mentions as single events, further reducing redundancy.


%%%%%%%%%%%%%%%%%%% START PREVIOUS VERSION %%%%%%%%%%%%%%%%%%%
% We first note that agreement between the annotators, as presented in Tables~\ref{tab:annot_agree}, is notably high across these tasks, indicating that our annotation tool effectively assists in generating high-quality annotations, while also ensuring completeness and consistency.
% From Table~\ref{tab:annot_time}, it is evident that annotating temporal relations is the most time-consuming task, requiring each annotator an average of 44.3 minutes to complete one document, while causal relations require 17.3 minutes, and coreference - 7.7 minutes. Table~\ref{tab:annot_step} indicates that \App{} assists in reducing complexity for temporal annotations by an average of 56\%, making the task feasible at this scale, and for causal annotations by 41\%. This reduction in causal annotation, combined with the EventStoryLine annotation scheme \cite{caselli-vossen-2017-event}, significantly expedites and simplifies the annotation process.
% \\~\\
% Overall, our annotation process produces complete and consistent graphs covering temporal, causal and coreference relations while maintaining simplicity. Using transitive closure algorithms significantly reduced the manual workload in temporal relation annotation by 56\%. This algorithm also help in preventing inconsistency errors in the generated data.
% Additionally, we choose the EventStoryLine approach for causal relation annotation after finding it superior to the RED approach in terms of inter-annotator agreement, indicating greater efficiency and simplicity (our experiments with both schemes are further detailed in Appendix~\ref{app:cause-scheme-expr}). 
% Finally, the task order further streamlined the process. Beginning with temporal relation annotation allowed subsequent steps to focus only on the relevant subset of pairs, leveraging the time constraint between temporal and other relations. This was particularly effective for coreference annotation, where the workload was reduced by 95\%. Additionally, annotating coreference before causal relations enabled us to treat coreferring event mentions as single events, further reducing redundant and preventing inconsistent annotations.
%%%%%%%%%%%%%%%%%%%%%% END PREVIOUS VERSION %%%%%%%%%%%%%%%%%%

%For coreference and causal annotations, coreference tasks are typically completed quickly due to the smaller number of relations needed for annotation. In contrast, causal annotations involve a much larger set of relations (as discussed in §\ref{tool:annot-flow}). While our tool achieves a 20\% reduction in complexity, the EventStoryLine annotation scheme \cite{caselli-vossen-2017-event} significantly simplifies this task.

%Finally, we observed disparity in performance among annotators. For instance, while annotator B completed the task in 76 minutes, annotator C took 111 minutes and made more temporal annotation steps, also showing lower agreement with others. This indicates that C struggled more with decision-making and may require additional training.

%For temporal annotation, annotators considered, on average, 15.2 mentions per document, totaling 228 mentions. The complete temporal graph would have required each annotator to annotate 1,635 pairs; however, less than 40\% of these relations required actual annotation to receive the complete graph. This indicates that the transitive closure and annotation flow significantly reduce the annotation complexity. Overall, annotators spent an average of 45 minutes annotating each document for temporal relations, and achieved 0.72 Cohen Kappa agreement, which is considered to be high agreement for this task.

%unlike the RED approach, it is inherently non-transitive,\footnote{The justification for this can be further explored in the original paper} thus avoids inconsistency risks.

==> backup/tool_before_rev.tex <==
\section{The \App{} Tool}
\label{tool}
\App{} is a web-based application designed specifically to assist annotators in the complex task of exhaustively annotating event-event relations in text documents, shown in Figure~\ref{fig:figure1}. 
In this section, we first describe the workflow of our annotation tool (§\ref{tool:annot-flow}). Then, we describe how we address the challenges of complexity, completeness and consistency, while maintaining high agreement among annotators (§\ref{tool:logic}). Lastly, we review the main features of the tool (§\ref{tool:feat}).

\App{} employs a layered annotation approach that breaks down the complex task of annotation into smaller, more manageable sub-tasks, with each step directly impacting the following steps. 
% Each step builds upon the decisions made in the previous step (§\ref{tool:logic}).
Specifically, \App{} consists of four steps, each accompanied by designated instructions (§\ref{back:annot-schemes}), illustrated in Figure~\ref{fig:figure1}.

% by instructions (adheres to the annotation guidelines described in §\ref{back:annot-schemes}), and provided with the document text, the highlighted events to consider and a straightforward questions that annotators are required to answer. 


\subsection{Event Selection}
\label{tool:annot-flow}
The first step in the annotation process involves selecting the set of events that will form the nodes of the event relation graph (Step 1 of Figure~\ref{fig:figure1} and Figure~\ref{fig-appx:select}). Prior to this step, all event mentions are extracted from the text using the \cite{cattan-etal-2021-cross-document} event detection model.

Following the Multi-Axis \cite{ning-etal-2018-multi} annotation methodology, the annotator is presented with an event and must determine whether the event actually occurred or will definitely occur (``anchorable in time''), or if it did not actually happen (e.g., events that are intentional, hypothetical, recurring, etc.).

All event mentions selected as actual will be considered in the following steps (\alone{ref to subsections}), while all other events will be excluded from the annotation process.

% The rationale for this selection is detailed in §\ref{appx:event-sel}.

%First, as shown in Step 1 of Figure~\ref{fig:figure1} and Figure~\ref{fig-appx:select}, annotators are required to assign each event mention (sequentially) in the provided text to its corresponding logical timeline \emph{axis}. In subsequent annotation steps, only those events designated as actual events (e.g., the main axis) will be considered, while all other events will be excluded from the annotation process.
% The rationale for this selection is detailed in §\ref{appx:event-sel}.

\subsection{Temporal Annotation}
The next step involves \emph{temporal} relation annotation (Step 2 of Figure~\ref{fig:figure1} and Figure~\ref{fig-appx:temporal}). Here, annotators are presented each time with two event mentions and are tasked with deciding which started first.
% and are required to answer \emph{which event started first?} then choose the most appropriate answer from four options corresponding to the four temporal relations considered in this scheme: before, after, equal, or uncertain.


\subsection{Coreference Annotation}
The next step involves \emph{coreference} annotation, as detailed in Step 3 of Figure~\ref{fig:figure1} and Figure~\ref{fig-appx:coref}. In this step, annotators are presented with an event mention, and the set of event mentions labeled with an \emph{equal} time relation to it.
%In this step, annotators are presented with an event mention in focus, along with a set of candidate event mentions that were annotated with an \emph{equal} time relation to it in the previous step. 
The annotators are then tasked with determining \emph{which events refer to the same event in focus?} All selected event mentions will then form a cluster.

\subsection{Causal Annotation}
The final step involves \emph{causal} relation annotation, as depicted in Step 4 of Figure~\ref{fig:figure1} and Figure~\ref{fig-appx:causal}. Similar to the coreference step, annotators are presented with an event mention, the set of all event mentions labeled as preceding it. Annotators are required to determine \emph{Why did the event happen?}. All selected event mentions will be labeled as causing events, and all others as none-causing relations.


\subsection{Ensuring Completeness, Consistency and Reduced
Complexity}
\label{tool:logic}
% 1) Selecting the annotation step sequence to benefit from the temporal constrain
% 2) Within each relation we select an annotation scheme which is simple to annotate and provide high agremeent
% 3) Apply algorithms that ensure transitive both in the events selection in temporal relation and fill in the other relations.

Facilitating the annotation of a complete event-event relation graph, including temporal, coreference, and causal relations, is challenging. First, we selected annotation schemes that ensure two key attributes: support exhaustive annotation between all events, and simplify the annotation to increase agreement (§\ref{back:annot-schemes}).

However, to make annotation feasible, it is essential to manage the quadratic annotation complexity of each relation type while ensuring the resource is complete and consistent (§\ref{back:compl-consist-complex}). 
Given the high number of pairs requiring consideration for each relation type, it is unrealistic to expect annotators to adhere perfectly to these three constraints. To accomplish this, \App{} provides a supportive framework that aids annotators in their tasks. This framework leverages the two levels of granularity required for this type of annotation: (1) across the different tasks, and (2) within each specific required annotation task.

% To make this annotation feasible and ensure its high quality, we integrate methodologies and algorithms specifically designed for annotating event-event relations from end to end. Our objective is to simplify the annotation process by reducing complexity and cognitive load on annotators, while ensuring the completeness and consistency of the annotations (§\ref{back:compl-consist-complex}). 

\paragraph{Across Tasks}
Starting the relation annotation with the temporal task is strategic, as it allows for leveraging the temporal constraints (as detailed in §\ref{back:event-rels}) in subsequent coreference and causal annotation steps.
For the succeeding coreference task, annotators are presented only with candidate pairs previously annotated with an \emph{equal} temporal relation. This approach is based on our observations and those reported in prior work \cite{ogorman-etal-2016-richer, wang-etal-2022-maven, rogers2022narrativetime}, where \emph{equal} relations constitute about 5\% of all relations. Thus, considering only event mentions with an \emph{equal} relation dramatically reduces the annotation complexity in this step.
Ending the task with the causal annotation step was strategically planned as well. Initially, only event mentions that have been previously identified with an \emph{after} or \emph{before} temporal relation are considered. Additionally, by leveraging the selections made during the coreference step, where event mentions are clustered, we can treat each cluster as a single event. This method effectively reduces redundancy and potential inconsistencies. 
Consequently, this approach decreases the complexity involved in annotating causal relations by approximately 20\%, as detailed in Table~\ref{tab:annot_step}.

\paragraph{Temporal Relation}
In this step, annotators are tasked with identifying the appropriate temporal relation between pairs of event mentions (§\ref{tool:annot-flow}). Given that each pair of events must be classified into one of four temporal relations, achieving comprehensive temporal annotation is considered the most challenging among the three types of event-event relations. 

To facilitate this process, \App{} guides the annotator through the annotation using a sequential pairwise method, while a transitive closure algorithm (further detailed in §\ref{appx:transitive-constraints}) runs in the background to build transitive relations. 

For example, with three mentions labeled {A, B, C} (by their appearance order in the text), the annotator is first presented with the pair A and B. Subsequently, the pair B and C is presented. This order is chosen because if (for example) A is annotated as \emph{before} B, and B as \emph{before} (or \emph{equal}) C, then it can be transitively inferred that A is also before C, thus A and C can be automatically annotated. \App{} will only present A and C if their relation cannot be inferred transitively.

This method significantly reduces redundancy by avoiding unnecessary annotations. In our pilot study (§\ref{pilot:results}), we demonstrate that this approach reduces the complexity of temporal relation annotation by about 60\%.

Another challenge in the temporal annotation process involves identifying relations that are inconsistent or contradictory to previously made annotations. For instance, consider an annotation where $A$'s relation to $B$ is marked as \emph{uncertain}, and $B$ is annotated as \emph{after} $C$. In such a scenario, the relation between $A$ and $C$ is undetermined and thus is flagged by the tool for further annotation. Should the annotator then designate $A$ as \emph{before} (or \emph{equal}) to $C$, a contradiction emerges: the inferred transitive relation from $A$ to $B$ (through $C$) would suggest \emph{before}, clashing with the directly annotated \emph{uncertain} relation between $A$ and $B$. 

As discussed in §\ref{back:compl-consist-complex}, this is not always monitored. Alerting annotators to resolve these inconsistencies plays a critical role in preserving annotation quality and increasing agreement (for more details about our discrepancy algorithm see §\ref{appx:discrepancy}).


\paragraph{Coreference Relation}
By limiting our focus to only \emph{equal} relation in this step, we effectively manage complexity. To manage quality, we utilize transitive closure tailored for coreference (§\ref{appx:coref}), and perform discrepancy checks to identify when annotators select the same mention to exist in two separate cluster of non-coreferring events.

\paragraph{Causal Relation}
The causal relation poses significant challenges due to two main factors. First, the high number of \emph{before/after} relations that require annotation. Second, the limited applicability of causal transitivity means that there is minimal complexity reduction from transitive relations (further detailed in \ref{appx:cause}).

To address this complexity, we experimented with various annotation schemes, ultimately focusing on RED and EventStoryLine (§\ref{back:annot-schemes}), to guide our annotation of causal relations.

Our findings indicated that annotating causality using the RED methodology required more than twice the time compared to the EventStoryLine methodology. This discrepancy arises because the number of annotation steps in RED is quadruple, covering all pairs, whereas EventStoryLine is linear, covering all events. 

Additionally, we observed that in the EventStoryLine scheme, annotators could quickly dismiss irrelevant candidates from the list. In contrast, within the RED scheme, annotators often struggled to decide whether the tail event was inevitable given the head event, even with clear causal indicators in the text. For example, in the sentence ``He answered the phone \emph{because} it rang,'' it was challenging for annotators to ascertain whether answering was inevitable or not.

Finally, The EventStoryLine causal methodology is non-transitive,\footnote{The justification for this can be further explored in the original paper \cite{caselli-vossen-2017-event}} thus ensuring consistency and completeness.

Overall, we observed that using EventStoryLine led to much higher agreement among annotators and required half the time to annotate.


\subsection{\App{} Features}
\label{tool:feat}
We incorporated several features into \App{} designed to help annotators navigate, keep track of, and visualize their progress while annotating. This, while making an effort to maintain a simple user interface (UI) that does not require extensive training to operate.

\paragraph{Task Navigation} \App{} consists of three navigation button types. The first two button types are designed to help annotators navigate through the annotations of the task currently presented to them: (1) \emph{Next/Prev} buttons allow users to sequentially navigate through all annotation candidates, completed and pending. (2) The \emph{Next Unhandled Pair} button directs the annotator to the next required annotation candidate, ensuring that all potential candidates are addressed, and in the required order to reduce redundant annotations. Once there are no more unannotated candidates, a message indicating task completion will appear. 

(3) The third button type, \emph{Next/Prev Task}, enables annotators to move between the different tasks, allowing them to proceed to the next task when there are no more unhandled candidates in the current task, and to revise annotations from previous tasks as they deepen their understanding of the text through their progression in the annotation process. At the last task, this button will change to \emph{Done?}, assisting annotators in verifying the completion of the entire annotation process. 


\paragraph{Graph Visualization} This feature provides annotators with a graphical representation of events and their relationships (Figure~\ref{fig-appx:temporal}), significantly enhancing the event-event annotation experience. The graph serves a dual purpose: first, as a visual representation of the annotations at each step. Second, in the temporal annotation step, it allows the annotator to manually pick a pair to annotate. 




\avivs{after all subsections, do a separate paragraph/subsection about the overall objectives met.}


==> backup/tool_text.tex <==
%In this work, our goal is to develop a dedicated tool for comprehensive annotation of event-event relations. To make this annotation feasible and ensure its high quality, we integrate methodologies and algorithms specifically designed for annotating event-event relations from end to end. Our objective is to simplify the annotation process by reducing complexity and cognitive load on annotators, while ensuring the completeness and consistency of the annotations. 

%\App{} takes as input a text document where event mention candidates have already been identified,\footnote{For our pilot study (§\ref{pilot}), we used the event detection model from \citet{cattan-etal-2021-cross-document}, although any event detection model can be utilized for this preliminary step.} 
%\avivs{If you say what the tool takes as input, you should also mention what is the expected output.}

%This design is primarily aimed at reducing the cognitive load on annotators and incorporate the temporal constrains learned at each steps to the next step, thus further minimizing the total amount of annotations required.
%Annotating all relations between all events in a document is a very challenging task (as described in §\ref{back:annot-schemes}). To mitigate this, unlike prior work which often limited annotations to relations between adjacent sentences, or short documents. In this work, we aim to establish all relations between a set of predefined event mentions.

%Subsequently, we only advance event mentions that are selected on the \emph{main} axis to the next steps (the rationale for this is detailed in §\ref{app}). This approach helps limit the scope of the annotation to a manageable set of mentions.

% among four relations types—\emph{before}, \emph{after}, \emph{equal}, or \emph{vague}—focusing solely on the events' starting times (further discussed in §\ref{appx:start-time}). 

%To facilitate this, \App{} guides the annotator through the annotation process, as further detailed in §\ref{tool:logic}.

%It is worth nothing that in our experiments, as well as in prior work \cite{ogorman-etal-2016-richer, wang-etal-2022-maven, rogers2022narrativetime}, the \emph{equal} relations constitute about 5\% of relations. Thus, considering only event mentions with \emph{equal} relation reduces the annotation complexity in this step dramatically. 

%We designed this step in accordance with the traditional coreference chains annotation methodology (§\ref{back:annot-schemes}). All selected event mentions will form a cluster. Events that do not share an equal relation with any other event mention, or are not selected by the annotator to be part of any cluster, will be labeled as singleton clusters.

%Given that most relations are \emph{before} and \emph{after} relations, the causal annotation steps introduce significant complexity. To address this challenge, we follow the EventStoryLine annotation scheme (§\ref{back:annot-schemes}), which helps reduce complexity and annotation time while increasing agreement among annotators.

%\cite{cybulska-vossen-2014-using}. Here, the annotator must select from a set of mention candidates which ones corefer (or belong to the same cluster) with the focused event mention (as illustrated in Step 2 Figure~\ref{fig:figure1}, and in Figure~\ref{fig-appx:coref}). 

%The annotator will then be presented with the next event (which represent the cluster), along with the event mention candidates that share an equal time relation with it. 

%We consider this assumption a robust alternative to the traditional TimeML \cite{pustejovsky2003timeml} methodology (which anchor events to time expressions).\footnote{\App{} focuses exclusively on the main axis, as further detailed in Appendix~\ref{appx:event-select}.}

%After selecting the main events, the next step is the \emph{temporal} relation annotation (step 2 in Figure~\ref{fig:figure1}), which focuses on identifying the main axis's triggering event for those identified as intentional events in the previous step. Those two steps help in filtering irrelevant events as well as constructing the three main axes that play a role in the annotation. .


%To that end, \App{} consist of five main steps (illustrated in Figure~\ref{fig:figure1}), each step is guided through instruction (\alone{point to instructions in appendix}) and simple questions that the annotator is required to answer to make informed annotation decisions. The initial three steps adhere to the MATRES \cite{ning-etal-2018-multi} methodology (see~\ref{back:coref-cause-temp}). First (step 1 in Figure~\ref{fig:figure1}), the annotator is required to assign each event to its corresponding \emph{axis} (main, intentional, hypothetical), or determine whether the event should be filtered (recurring, negations, not-event, etc.). This is followed by the \emph{anchoring step} (step 2 in Figure~\ref{fig:figure1}), which focuses on identifying the main axis's triggering event for those identified as intentional events in the previous step. Those two steps help in filtering irrelevant events as well as constructing the three main axes that play a role in the annotation. According to the MATRES methodology, relations are permissible only within the same axis.

%The first two steps follows the MATRES methodology (see \ref{back:coref-cause-temp}) and are design to designate each event to its relevant axis (i.e., main, intentional, hypothetical), as well as event that should not be annotated as they are (recurring, negations, abstract, or not events) followed by an anchoring step to identify the triggering events on the main axis of all events selected as intentional events. Those two steps help in filtering irrelevant events as well as construct the three main axis that play a role in the annotation, and the event pairs that should be presented to the annotator according to the MATRES methodology of possible relations between events on different axis.

%Since any pair of relations should have a temporal relation, achieving a complete temporal annotation is considered the most challenging among the three event-event relation types. To be able to achieve such annotation, The \App{} guide the annotator trough the annotation process as further detailed in §\ref{tool:logic}. 

%\footnote{In our experiments and as well in prior work \cite{ogorman-etal-2016-richer, wang-etal-2022-maven, rogers2022narrativetime}, the before and after relations constitute about 95\% of the non-vague relations, thus, in the coreference step, only 5\% of the none-vague relations will be presented.} 

%where only candidate event mention pairs annotated with a \emph{before} or \emph{after} time relation are considered. This approach is based on the premise that an event causing another must have occurred first. 


%For temporal annotation, we have implemented an algorithmic framework that significantly reduces the number of steps required, as illustrated in the table \alone{ref to annotation steps done table} and further discussed in §\ref{tool:logic}. To manage the causal relation, we leverage temporal annotations to present only \emph{before/after} pairs and utilize coreference annotations to present only a representative event from each cluster, rather than all events within the cluster. This strategy reduces the number of pairs requiring annotation. However, since the transitive closure of causal relations is much more stringent (See Appendix~\ref{fig-appx:temporal}), the capability of the transitive algorithm to reduce complexity is rather limited, and the annotation challenge remains significant.


%we adopt the annotation methodology from EventStoryLine \cite{caselli-vossen-2017-event},\footnote{We only consider the causal relation (without enablement), similar to \citet{ning-etal-2018-joint, do-etal-2011-minimally}.} where each event is presented with all preceding events. The annotator needs to determine \emph{why the event in focus has happened} and then verify if the causal event is among the listed candidates. This in contrast to the RED \cite{ogorman-etal-2016-richer} annotation methodology, where given an event pair, involves assessing if \emph{the tail event is inevitable given the head event}. 

%We experimented with both methods and found that the approach by \citeauthor{caselli-vossen-2017-event} significantly reduces annotation time, and complexity, while increasing the agreement among the annotators. First, the number of annotation steps required is decreased from quadruple (all pairs) to linear (all events). Second, since most of the preceding event candidates can be quickly dismissed as irrelevant, decision-making requires only the investigation of a few (to none) relevant events among the candidates. 

%In our experiments, annotating causality using the RED methodology presented two significant challenges. First, it required more than twice the time compared to the EventStoryLine methodology. Second, annotators faced difficulties in deciding whether the tail event was inevitable given the head event, even when causal indicators were present in the sentence. For example, in the sentence ''He answered the phone because it rang,`` it is challenging to ascertain whether answering was inevitable.

%Our experiments demonstrate that this significantly reduces the cognitive load, annotation time and complexity (\alone{ref to table or section}), as most candidates can be quickly dismissed, leaving only a few relevant ones that require further textual analysis to determine.

%Subsequently, the annotator is sequentially moved to the next event mention in the text. As illustrated in Table \alone{ref to table with time measure}, the combination of this approach with our flow and pair reduction strategies significantly reduces the annotation time and the number of steps required for the causal relation annotation while supporting high annotation agreement (as illustrated in Table~\alone{add IAA table and ref to it}).


%Each step within the tool is accompanied by comprehensive annotation guidelines, including examples that annotators can reference as needed during the annotation process. Furthermore, the system is highly configurable: annotation administrators can select which annotation steps to include and which axes to consider (for instance, some of the previous work only considered events placed on the main axis, ignoring events marked on other axes). The software is also designed with modularity in mind, making it easy to incorporate new logic, steps, or relationships into the workflow.

%Three main motivations guided the development of our annotation tool: (1) Ensuring annotation \emph{completeness} by identifying pairs of events that require annotation. (2) Reducing annotation \emph{complexity} by streamlining the annotation process for annotators, presenting only the necessary and missing relations to annotate, while skipping any relations that can be indirectly inferred (transitively). (3) Ensuring \emph{consistency} by identifying and notifying annotators of any contradictory relations (inferred directly or indirectly).

%\subsubsection{Transitive Closure Algorithms}
%\label{logic:trans-closure-algo}
%Temporal, coreference and causal relations each have a unique transitive closure use-case for which we developed a novel and specific algorithm to aid in the annotation process while it is performed.

%Matrix \(X\) is shared across all types of relations and annotation steps, maintaining a record of both applied and required annotations. To support this, we have created distinct representations for each subtype of the temporal, causal, and coreference relations within matrix \(X\). Additionally, we have integrated appropriate rules within the Warshall algorithm to accommodate these distinctions.\footnote{Further details of our implementation can be seen in \url{https://github.com/AlonEirew/EventGraphAnnot/blob/main/public/objects/graph_algo.js}}.


% \paragraph{Temporal Transitive Closure}
% Being able to deduce the transitive relation in a temporal graph is a challenging task that was mostly explored in the temporal annotation scheme of Allen relations \cite{allen-et-al-1983} and TimeML \cite{pustejovsky2003timeml}. Since our annotation scheme follow a more narrow scheme covering a subset of four temporal relations (after, before, equal, vague), we developed a novel temporal algorithm inspired by \cite{ALLEN1984123, VILAIN1990373, setzer-2002-temp, pustejovsky2003timeml}, for supporting both annotation completeness and consistency by leveraging the transitive relations while annotation is being performed.

% \paragraph{Coreference Transitive Closure}
%Coreference is the relation that indicates whether two events mentioned in text are in fact two mentions of the same real world event. Due to this, there is a strong constrain indicating that only an equal time relation might exist between such two event mentions (as any other temporal relation will contradict they are the same event). Thus, in our annotation scheme, since temporal relations are the first step of the annotation procedure, at the step of coreference annotation, we only present pairs of events with equal time to the annotator to determine whether they corefer or not. 
%Following this, the transitive closure for the coreference relations, will only consider events that can be reached transitively with a path of equal time relations. Then, given two events without a direct path, in case the indirect path was already annotated with coreference relations, the coreference transitive closure algorithm will examine if a transitive relation of either coreference or not-coreference can be inferred. In the case that it cannot be inferred, we prompted the user with the pair to be annotated (for more details see Appendix~\ref{appx:coref-closure-algo}).

%One approach to mitigate this issue is by preventing annotators from making such annotations in the first place. This preventive measure is facilitated through the ''Next Unhandled Pair`` and ''Graph Visualization`` features, as detailed in Section~\ref{method:feat}. 

%Nevertheless, situations may still arise where an annotator needs to annotate a pair whose transitive relation is ambiguous. 

%Our annotation methodology is constructed with the thought of mitigating discrepancy as much as possible, the process of annotating first the temporal relations following by the coreference and causal relations by allowing annotation to pairs of nodes with  temporal relation that consent with the relation temporal constrains (equal in case of coreference and before/after in case of caused/caused-by), insure that in the causal and coreference relations no contradicting between temporal and underline causal or coreference relation might exist.

%To that end, we constructed a set of rules (\alone{ref to appendix}) that ensure no such contradiction is made. In case the algorithm find contradicting relations, an alert will be presented to the annotator indicating the event pair, the direct relation and the contradicting inferred relation.

%Given the extensive scope of the tasks, it is crucial to have a mechanism that ensures no part of the process is overlooked. If there are missing annotations, clicking the button will navigate the annotator to the specific task and highlight the missing annotation.

%This is useful when an annotator identifies relationships that he would like to already annotate or revise.

%Furthermore, to ensure annotation consistency, if an annotator attempts to manually select a pair for annotation whose underlying temporal relation contradicts the intended annotation, for instance, selecting a pair with a 'before' temporal relation during a coreference annotation step, an alert is generated to indicate that the selected pair is incompatible with the intended relation.

%In some cases, particularly when handling many events and ambiguous relationships, it may become difficult to interpret the graph as it becomes dense \alone{Find a citation for this}. To maximize the graph viability for the user, only the edges that are relevant in the current step will be highlighted, hiding any irrelevant edges (see Figure~\ref{fig-appx:coref} and Figure~\ref{fig-appx:causal}).

%However, as the annotator progress in the annotation, the graph visualization can become quite dense with relations which make it rather useless to the annotator both in the visual aid and in selecting pairs to annotate. Additionally, prior work allowed the user only to annotate relations through the graph by picking two nodes and drawing a line between them (\alone{Make sure this is right + cite papers}).

%To that end, we integrated few features in the graph visualization to make it viable throughout the annotation steps. (1) As mentioned above, we allow the annotator to navigate using the next unhandled pairs, and we also provide the annotator with the chooise of selecting nodes from the graph to annotate. This is helpful when the annotator identify relations that he would like to already annotate and not wait to reach them sequentially through the pair suggestion option. (2) We remove redundant transitive closure edges while annotation is performed to ease relations that can be deduced and therefor remove to ease the load on the graph. (3) We highlight only the edges that are relevant to the current step, and hide irrelevant edges. For Example, in the coreference step, only relations with temporal edge that are \emph{equal} are relevant, thus we hide the rest of the edges (e.g., before, after and vague). 

% \subsection{Annotation Methodology}
%\alone{Here I need to describe that because this is a dense graph, if two annotators make different decisions this might reflect the next annotation steps, and without consolidation annotators will annotate different set of relations with the coref and causal relation making the annotation unstable and hard to maintain. Here we explain how we propose to handle this scenario}.



==> backup/tool_v2.tex <==
\section{The \App{} Annotation Tool}
\label{tool}

%\App{} is a web-based tool designed to annotate \textit{complete} and \textit{consistent} event relation graphs over a manageable subset of ``anchorable in time'' events, encompassing temporal, coreference, and causal relations (Figure~\ref{fig:figure1}). It accepts a document with pre-identified event mentions, obtained from any off-the-shelf event extraction model, along with an optional set of extracted temporal entities.\footnote{The input document structure is provided in simple JSON format, with details available in our Git repository.}


This section outline the annotation protocol that annotators follow at each annotation step (§\ref{tool:annot-schemes}), followed by a detailed explanation of the \App{} tool workflow (§\ref{tool:annot-flow}).

\subsection{Annotation Scheme Output}
\label{tool:annot-schemes}

\paragraph{Event Selection and Temporal Relation} 
To select a subset of event mentions where a temporal relation can be established between any pair across the entire document, we adopt the Multi-Axis \cite{ning-etal-2018-multi} annotation method. First, this method distinguishes event mentions by their temporal characteristics—those that are actual or ``anchorable in time'' (e.g., they \textit{\underline{won}} the game) and those that are not, such as wishful, intentional, or conditional events (e.g., I wish they \textit{\underline{win}} the game). This selection ensures that all selected events can be placed on a timeline and related through temporal relations.

Next, the Multi-Axis method defines four temporal relation types: \textit{before}, \textit{after}, \textit{equal}, and \textit{vague}, focusing on the start times of events.\footnote{The inclusion of end times has proven challenging for annotators and often results in low agreement levels.} Notably, the \textit{vague} relation is crucial for annotating complete temporal graphs and improving agreement, as it accounts for relations between events that cannot be resolved from the given context.


\paragraph{Coreference Relation} 
We adopt the traditional coreference chains annotation methodology \cite{cybulska-vossen-2014-using, ogorman-etal-2016-richer}, where annotators cluster event mentions referring to the same real-world event into coreference clusters. Coreferring events can often be identified by observing shared arguments between events (e.g., location, participants, etc.). Event mentions that do not corefer with any other mentions are marked as singleton clusters.


\paragraph{Causal Relation} 
% Annotating causal relations typically adheres to the RED protocol \cite{ogorman-etal-2016-richer}, which involves evaluating all event pairs, adding significant complexity. In contrast, 
We adopt the EventStoryLine methodology \cite{caselli-vossen-2017-event},\footnote{We focus exclusively on the causation relation, excluding enablement and prevention, similar to \citet{do-etal-2011-minimally, ning-etal-2018-joint}.} presenting an event alongside \emph{all} its preceding events and asking annotators to identify the causing event(s). Since the \textit{before} relation constitutes about 85\% of all temporal relations, this simultaneous consideration of preceding events — rather than pairwise evaluation as used in other annotation approaches, such as the RED methodology \cite{ogorman-etal-2016-richer}, reduces cognitive load and supports high-quality annotation. Our experiments further demonstrate its effectiveness.\footnote{Details in Appendix~\ref{app:cause-scheme-expr}.} Notably, the EventStoryLine method treats causal relations as non-transitive and localized, reducing the need for transitive consistency required in other relation types.


\subsection{Annotation Workflow}
\label{tool:annot-flow}
In this section, we detail the workflow and usability of the four-step annotation process in \App{} (illustrated in Figure~\ref{fig:figure1}).

\App{} is a web-based tool designed to guarantee \textit{complete} and \textit{consistent} event relation annotations over a manageable subset of events. It encompasses temporal, coreference, and causal relations (Figure~\ref{fig:figure1}) within a unified framework and aims to reduce the overall annotation workload. 

\App{} employs a layered annotation approach over the provided set of events, dividing the annotation process into four sub-tasks: event selection, temporal relations annotation, coreference annotation, and causal relations annotation. Each task includes detailed guidelines and instructions (see examples in Appendix~\ref{appx:guidelines}) to assist annotators in managing the process (see printscreens of \App{} in Appendix~\ref{appx:additional_printscreens}). At each task, annotators can save their progress, and upon completing all tasks, the final annotation can be exported as a JSON file.

The annotation process begins with a document containing pre-identified event mentions, obtained from any off-the-shelf event extraction model, along with an optional set of extracted temporal entities.\footnote{The input document structure is provided in simple JSON format, with details available in our Git repository.}

\input{latex/tables/disc_temp}


\paragraph{Event Selection Step}
The annotation process begins with a document containing pre-extracted highlighted event mentions, from which annotators identify ``anchorable in time'' mentions (§\ref{tool:annot-schemes}) (illustrated in Appendix~\ref{appx:additional_printscreens}, Figure~\ref{fig-appx:select}). Only these anchorable event mentions proceed to subsequent steps. For large documents with a substantial set of anchorable events, temporal relation annotation becomes less manageable for non-expert annotators, requiring a narrower set of event mentions. In such cases, annotators focus on the most significant events relevant to the downstream task (e.g., most salient events in a topic).\footnote{In our experiment, selecting more than 20 events proved challenging for non-expert annotators.}


\paragraph{Temporal Relation Annotation Step}
The next step involves annotating \emph{temporal} relations (illustrated in Appendix~\ref{appx:additional_printscreens}, Figure~\ref{fig-appx:temporal}), with the goal of establishing links between \textit{all} pairs of event mentions selected in the previous step. Annotators review these pairs within their context, presented one at a time, where one event is marked in red and the other in green. Temporal entities, if extracted, are also highlighted. Alongside this, a visualization of the updating relation graph is provided, with the scrutinized pair emphasized. Annotators must determine whether one of the events started first, if both started simultaneously, or if the timeline is uncertain. Notably, the graph visualization aids in tracking progress and enhances flexibility, allowing annotators to directly select and annotate (or fix) pairs by clicking on the corresponding graph nodes.

\begin{figure}[t!]
\centering
\includegraphics[width=0.48\textwidth]{latex/figures/example1.png}
\caption{A simple example illustrating the prioritization strategy and automatic annotation of transitive relations. The tool sequentially presents the pairs \textit{`accident-collided'}, \textit{`collided-damage'}, and \textit{`damage-responded'} based on the annotator's selected relations, automatically annotating in the background the relations for \textit{`accident-damage'}, \textit{`accident-responded'}, and \textit{`collided-responded'}.
}
\label{fig:example}
\end{figure}


To ensure completeness and consistency (§\ref{back:compl-consist-complex}), all event pairs must be annotated without contradictions. 
% Given the large number of pairs, expecting annotators to perfectly comply with these standards is unrealistic. 
To address this, \App{} uses a transitive closure algorithm \cite{ALLEN1984123} inspired by \citet{ning-etal-2018-joint} temporal constraints (Table~\ref{tab:disc_temp}), applied after each annotation. This algorithm identifies and \textit{auto}-annotates unhandled pairs whose links can be transitively deduced from already annotated pairs (scenarios 1-7 in Table~\ref{tab:disc_temp}), thereby reducing the number of pairs requiring \textit{manual} annotation (scenarios 8-16 in Table~\ref{tab:disc_temp}). To optimize the algorithm's effectiveness, \App{} uses a prioritization strategy activated after each relation selection. For example, in Figure~\ref{fig:example}, once the pair \textit{`collided-damage'} is annotated as \textit{BEFORE}, the ideal next pair is \textit{`damage-responded'}. This choice maximizes the likelihood of automatically discovering a transitive relation, in this case, \textit{`collided-responded'}.\footnote{For more details, see Appendix~\ref{appx:prior-strategy}.} 
Finally, before presenting the next pair, \App{} ensures the graph state is consistent. In cases of contradictions, such as annotating \textit{`accident-damage'} as something other than \textit{BEFORE} (Figure~\ref{fig:example}), the tool highlights the discrepancy and guides the annotator in resolving it. Once completeness and consistency are achieved, a notification confirms no more pairs remain to be annotated.


% Finally, before presenting the next pair for annotation, \App{} ensures current graph state is consistent. In cases of contradicting relations, either in directly or transitively linked pairs—for example, in Figure~\ref{fig:example}—the tool prevents errors such as annotating the relation \textit{`accident-damage'} as something other than \textit{BEFORE}. In such cases, a notification highlighting the discrepancy is displayed to guide the annotator in resolving the issue. Once completeness and consistency are achieved, a notification indicates that no more pairs remain to be annotated.


\paragraph{Coreference Annotation Step}
The next step involves \emph{coreference} annotation (illustrated in Appendix~\ref{appx:additional_printscreens}, Figure~\ref{fig-appx:coref}). To reduce workload, this step only focuses on event-mention pairs labeled as concurrent in the previous step, as only these can potentially corefer. Here, annotators review a target event mention and its co-occurring mentions, alongside a graph visualization to monitor progress. They are required to identify which of the concurrent mentions corefer with the event mention in question, forming coreference clusters. Annotators then advances using a designated button (``Next Unhandled'') to the next unclustered event mention with co-occurring mentions. Upon completion of this step, event mentions not included in any cluster are marked as singleton clusters. Additionally, a discrepancy detection algorithm ensures consistency by notifying annotators of any event mention erroneously linked to multiple, non-coreferring clusters.
%Lastly, a relation graph visualization helps annotators track annotated relations, but unlike the previous step, it cannot be used to navigate to specific pairs.



\paragraph{Causal Relation Annotation Step}
The final \emph{causal} relation annotation step (illustrated in Appendix~\ref{appx:additional_printscreens}, Figure~\ref{fig-appx:causal}) involves annotators examining an event mention within its context, alongside all events identified as preceding it in step [2], to determine which event(s) caused the event in focus. As with previous steps, a relation graph visualization aids in tracking annotations, and a designated button allows annotators to navigate to the next event mention with at least one preceding event.

After completing this step, annotators can run a completion check on the entire annotation, prompting the system to verify the annotations and, if any are missing, direct annotators to address the missing relations from previous steps.


==> emnlp_sec/background.tex <==
\section{Background and Related Work}
This section overviews relevant research on event relation graphs, covering their structure and desired properties (§\ref{back:compl-consist-complex}), relation types and annotation schemes (\S\ref{back:annot-schemes}), and annotation tools (\S\ref{back:annot-tools}).

% \subsection{Event-Event Relations}
% \label{back:event-rels}
% The three main relations types considered by \App{} are: \textbf{Temporal}, for understanding the sequence of events over time \cite{do-etal-2012-joint}; \textbf{Causal}, for understanding how one event influences another in a story \cite{chaturvedi-etal-2017-story}; and \textbf{Coreference}, for identifying mentions of the same event in texts \cite{raghunathan-etal-2010-multi}.\footnote{An additional relation type often considered is the sub-event relation \cite{glavas-etal-2014-hieve}. However, it is beyond the scope of this work.} Importantly, the latter two relations are directly governed by the temporal relation, i.e., coreferring events occur at the same time and events that cause other events naturally occur before them.

\subsection{Event Relation Graph} 
\label{back:compl-consist-complex}
An event relation graph consists of nodes, which represent event \textbf{coreference} clusters, i.e., groups of event mentions referring to the same real-world event  \cite{raghunathan-etal-2010-multi}, and edges, which represent the relations between these clusters. These relations include \textbf{Temporal} \cite{do-etal-2012-joint}, which encode the sequence of events over time, and \textbf{Causal} \cite{chaturvedi-etal-2017-story}, which indicates how one event influences another.\footnote{An additional relation type often considered is the sub-event relation \cite{glavas-etal-2014-hieve}. However, it is beyond the scope of this work.} Importantly, temporal relations exist between \textit{any} two event mentions, as any event pair can be placed on a timeline, while causal relations are only identified between positively linked pairs. Moreover, both coreference and causal relations are directly governed by temporal relations, as coreferring event mentions co-occur by definition, while causative events naturally precede those they impact.

% \footnote{For causal relations, all positively-linked pairs.}
Creating an event relation graph requires ensuring the \textit{completeness} and \textit{consistency} of annotations \cite{marc-et-al-2005-temporal}, linking all event pairs without contradictions. However, annotating every temporal relation in an article is considered infeasible \cite{naik-etal-2019-tddiscourse}, and inconsistent annotations are common among human annotators, as seen in the TimeBank corpus \cite{pustejovsky-stubbs-2011-increasing}. Therefore, a primary goal of \App{} is to help annotators produce a consistent and complete event relation graph.
%Previous works  \cite{pustejovsky-etal-2003, cassidy-etal-2014-annotation} often lacked these standards, showing inconsistencies \cite{pustejovsky-stubbs-2011-increasing} and missing relations \cite{reimers-etal-2016-temporal, rogers2022narrativetime}. 
%Our experiments also revealed inconsistencies in the TCR \cite{ning-etal-2018-joint} and EventCausality  \cite{do-etal-2011-minimally} datasets. 

%%%%%%%%%%%%%%%%%%% START PREVIOUS VERSION %%%%%%%%%%%%%%%%%%%
% To create a \textit{complete} event relation graph, monitoring annotation \emph{completeness} and \emph{consistency} is crucial \cite{marc-et-al-2005-temporal}. This involves ensuring that a relation is established between each pair of events, when applicable, and that there are no contradictory relations. 
% %—either directly or transitively, or between relation types (e.g., a causing event occurring \emph{after} the affected event). 
% Previous works often failed to meet these requirements. For instance, in the notable TimeBank corpus \cite{pustejovsky-etal-2003}. \citet{pustejovsky-stubbs-2011-increasing} identified inconsistencies, while \citet{reimers-etal-2016-temporal} criticized it for missing many relations. 
% Similarly, in our experiments, we discovered a few inconsistencies in the TCR \cite{ning-etal-2018-joint} and EventCausality \cite{do-etal-2011-minimally} datasets across relation types (such as \emph{cause/after}). 
% One of our primary goals in developing \App{} is to ensure that the produced event relation graph is consistent and complete.
%%%%%%%%%%%%%%%%%%%% END PREVIOUS VERSION %%%%%%%%%%%%%%%%%%%%

%The three relations types considered by \App{} are: \textbf{Temporal}, for understanding the sequence of events over time \cite{do-etal-2012-joint}; \textbf{Causal}, for understanding how one event influences another in a story \cite{chaturvedi-etal-2017-story}; and \textbf{Coreference}, for identifying mentions of the same event in texts \cite{raghunathan-etal-2010-multi}.\footnote{An additional relation type often considered is the sub-event relation \cite{glavas-etal-2014-hieve}. However, it is beyond the scope of this work.} Importantly, the latter two relations are directly governed by the temporal relation, i.e., coreferring events occur at the same time and events that cause other events naturally occur before them.

\subsection{Event-Event Relations Schemes}
\label{back:annot-schemes}
Different annotation schemes have been proposed for each of the aforementioned relations.

\paragraph{Temporal Relation} 
% is essential for understanding the sequence of events over time \cite{do-etal-2012-joint}. A temporal relation always exists between two events, as any two events can be placed on a timeline; however, it is not always resolvable from the given text.
Prominent prior works, including RED \cite{ogorman-etal-2016-richer}, EventStoryLine \cite{caselli-vossen-2017-event}, and MAVEN-ERE \cite{wang-etal-2022-maven}, have adopted the TimeML \cite{pustejovsky2003timeml} annotation scheme to annotate relations between \textit{all} temporal expressions (e.g., dates and times) and events. However, \textit{exhaustively} annotating these connections is impractical due to its quadratic complexity, resulting in sparsely annotated datasets. Additionally, this approach does not account for situations where relations cannot be determined from the context, which may decrease inter-annotator agreement.

%Additionally, this approach does not account for relations that cannot be determined from the context, which may decrease inter-annotator agreement.

%Consequently, many recent works \cite{ning-etal-2018-joint, wang-etal-2020-joint} have adopted the Multi-Axis \cite{ning-etal-2018-multi} annotation guidelines, which focus solely on temporal relations between events.
% This scheme requires events within a document to be linked to time expressions (i.e., TimeX\footnote{Temporal expression mark-up for temporal entities} or the DCT\footnote{The document creation time}) to establish temporal relations. %Thus, an event that cannot be anchored to any explicit time expression in the text is not annotated. 
% However, time expressions are not always present, as writers prioritize advancing their story engagingly rather than detailing every aspect. Consequently, the TimeML approach often does not yield dense temporal relations \cite{cassidy-etal-2014-annotation, rogers2022narrativetime}.
%Readers can either infer the relation using common-sense reasoning, or in some cases, the relation is indeterminate from the text and should be marked as vague (indicating that it was investigated but could not be resolved). 
 
Since our goal is to support \textit{complete} temporal annotation only between significant events, we adopt the Multi-Axis annotation scheme \cite{ning-etal-2018-multi}. This method categorizes events based on their temporal characteristics—actual or ``anchorable in time'' (e.g., they \textit{\underline{won}} the game), hypothetical (e.g., if she \textit{\underline{wins}} the race), and intentional (e.g., he plans to \textit{\underline{adopt}} a dog), along with other categories that cannot be temporally anchored. Following \cite{wang-etal-2022-maven, alsayyahi-batista-navarro-2023-timeline}, we only focus on `anchorable' events. 
The Multi-Axis method identifies four specific temporal relation types: before, after, equal, and vague, focusing on the start times of events.\footnote{The inclusion of end times has proven challenging for annotators, often leading to low agreement levels.} Notably, the vague relation plays a crucial role in annotating complete temporal graphs and improving agreement, as it enables covering all relations, including unresolved ones.
Yet, even after limiting the annotation scope to only `anchorable' events, the quadratic complexity challenge remains. To address this, we develop \App{}.

% To support \textit{complete} temporal annotation, we adopt the Multi-Axis annotation scheme \cite{ning-etal-2018-multi}. This method categorizes events based on their temporal characteristics—actual or ``anchorable in time'' (e.g., they \textit{\underline{won}} the game), hypothetical (e.g., I wish I could \textit{\underline{fly}}), and intentional (e.g., he plans to \textit{\underline{adopt}} a dog), along with other categories that cannot be temporally anchored. Following \cite{wang-etal-2022-maven, alsayyahi-batista-navarro-2023-timeline}, we only focus on `anchorable' events. 
% The Multi-Axis method identifies four specific temporal relation types: before, after, equal, and vague, focusing on the start times of events.\footnote{The inclusion of end times has proven challenging for annotators, often leading to low agreement levels.} Notably, the vague relation plays a crucial role in annotating complete temporal graphs and improving agreement, as it enables covering all relations, including unresolved ones.
% Yet, even after limiting the annotation scope to only `anchorable' events, the quadratic complexity challenge remains. To address this, we develop \App{}.

%Yet, even after limiting the annotation scope to only `anchorable' events, annotating \textit{complete} relation graphs still suffers from quadratic complexity.


% The Multi-Axis method identifies three specific temporal relation types--before, after, equal--focusing on the start times of events,\footnote{The inclusion of end times has proven challenging for annotators, often leading to low agreement levels.} as well as a fourth `vague' relation, which enables a complete event relation graph annotation, by considering ambiguous relations.

%However, exhaustively annotating all \emph{actual} events remains a challenge. To address this, we developed \App{} to help reduce the annotation complexity, as detailed in §\ref{tool:temp}.


% The Multi-Axis method identifies four specific temporal relation types: before, after, equal, and vague, with an emphasis on the start times of events.\footnote{The inclusion of end times has proven challenging for annotators, often leading to low agreement levels.} Importantly, the vague relation plays a crucial role in developing a complete event relation graph and improving agreement, as it covers relations that are considered but remain unresolved.

%To determine the relationship between two events, A and B, annotators answer two yes/no questions: A1) if A started before B, and A2) if B started before A. Then map the answer as follows: A1=A2=yes$\rightarrow$vague, A1=A2=no$\rightarrow$equal, A1=yes, A2=no$\rightarrow$before, and A1=no, A2=yes$\rightarrow$after. Overall, these simplifications help achieve high agreement among annotators. 

%in three key ways: (1) Four types of temporal relations are considered: \emph{before}, \emph{after}, \emph{equal}, and \emph{uncertain}, as opposed to the seven TimeML relations. 
%This reduction includes the most critical temporal relations and provides the necessary framework for annotating coreference and causal relations, which are temporally constrained by the \emph{equal} and \emph{before/after} relations. 
%(2) Events are categorized into logical timeline \emph{axes} (as listed in step 1 of Figure~\ref{fig:figure1}), distinguishing actual events (main axis) from theoretical ones (other axes). Since establishing a timeline between events that occurred and those that did not is impractical, temporal relations are permitted only between events on the same axis. (3) Only the starting time of events is considered. 

%Overall, these simplifications helped achieve high agreement among annotators. Consequently, we have adopted this method in our tool (§\ref{tool}).
%To the best of our knowledge, \App{} is the first annotation tool to support this annotation methodology.
%previous temporal annotation tools adhere to the TimeML scheme \cite{cassidy-etal-2014-annotation, derczynski-etal-2016-gate, fulda-etal-2016}, while no existing tools follow the Multi-Axis guidelines.

% However, exhaustively annotating all \emph{actual} events remains a challenge. To address this, we developed \App{} to help reduce the annotation complexity, as detailed in §\ref{tool:temp}.

%is considered not feasible, due to the quadruple complexity challenge. In an attempt to address this and increase the density of temporal relations, various studies \cite{cassidy-etal-2014-annotation, minard-etal-2016-meantime, caselli-vossen-2017-event, ning-etal-2018-joint} annotated relations only between adjacent sentences.


\paragraph{Coreference} 
%is essential for identifying mentions of the same event in texts \cite{raghunathan-etal-2010-multi}. This task involves clustering coreferring event mentions into event clusters. In an event relation graph, these event clusters represent the nodes of the graph. 
\App{} adheres to the traditional coreference chains annotation methodology \cite{cybulska-vossen-2014-using, ogorman-etal-2016-richer}, where annotators cluster event mentions that refer to the same real-world event into coreference clusters. Event mentions that do not corefer with other mentions are marked as singleton event clusters. 
%Importantly, coreference relations are directly governed by the temporal relations and must satisfy the temporal co-occurrences relation, which is leveraged in our annotation flow.
% coreferring event mentions must occur at the same time.


\paragraph{Causal Relation} 
Annotating causal relations typically adheres to the RED protocol \cite{ogorman-etal-2016-richer}, which involves evaluating all event pairs, adding significant complexity. 
In contrast, we follow the EventStoryLine methodology \cite{caselli-vossen-2017-event},\footnote{We only focus on the causation relation (excluding enablement and prevention), similar to \citet{ning-etal-2018-joint, do-etal-2011-minimally}.} which unlike RED, presents an event with \emph{all} its preceding events, and asks annotators to identify the causing event(s) from these candidates. By considering all preceding events at once rather than evaluating each pair separately, this approach significantly reduces the cognitive load required for an exhaustive and high-quality annotation. This is further demonstrated in our experiments, where EventStoryLine achieved higher annotator agreement compared to RED.\footnote{Further detailed in Appendix~\ref{app:cause-scheme-expr}.}

%%%%%%%%%%%%%%%%%%% START PREVIOUS VERSION %%%%%%%%%%%%%%%%%%%
% To annotate causal relations, it is standard practice to follow the RED annotation guidelines \cite{ogorman-etal-2016-richer}, which require assessing all pairs of events, adding significant complexity. To simplify this process, we adopt the EventStoryLine methodology \cite{caselli-vossen-2017-event},\footnote{We only focus on the causation relation (excluding enablement and prevention), similar to \citet{ning-etal-2018-joint, do-etal-2011-minimally}.} which differs from RED by presenting an event alongside \emph{all} its preceding events, requiring annotators to select all the causing event(s) out of these candidates. Our experiments with both methods (Appendix~\ref{app:cause-scheme-expr}) show that the EventStoryLine method is more efficient and achieves higher agreement among annotators than the RED methodology. 
%%%%%%%%%%%%%%%%%%%%%% END PREVIOUS VERSION %%%%%%%%%%%%%%%%%%


% is essential for understanding how one event influences another in a story or narrative \cite{chaturvedi-etal-2017-story}. Unlike a temporal relation, a causal relation exists only between positively identified pairs; all other pairs are considered negative examples.


% Notably, causal relations are also directly governed by temporal relations; naturally, an event that causes another must precede it.


%Since our approach aims to reduce the quadratic annotation complexity necessary for achieving a complete event relation graph.  In contrast to RED, this methodology presents each tail event alongside \emph{all} preceding events. Annotators are tasked with determining \emph{why the tail event occurred} and identifying if the cause is among the listed candidates (head events). Our experiments (detailed in §\ref{app:cause-scheme-expr}) demonstrate that this method is more efficient and achieves higher agreement among annotators then the RED methodology. Notably, causal relations are also directly governed by temporal relations; naturally, an event that causes another must precede it.

%In contrast, the EventStoryLine methodology \cite{caselli-vossen-2017-event} presents each tail event alongside all preceding events. Annotators are tasked with determining \emph{why the tail event occurred} and identifying if the cause is among the listed candidates. Our experiments (detailed in §\ref{tool:logic}) demonstrate that this method is more efficient and achieves higher agreement among annotators. Therefore, we have adopted the EventStoryLine approach in \App{}.\footnote{We only consider the causal relation (without enablement), similar to \citet{ning-etal-2018-joint, do-etal-2011-minimally}.}

%For the causal annotation, we adopt the annotation methodology from EventStoryLine \cite{caselli-vossen-2017-event},\footnote{We only consider the causal relation (without enablement), similar to \citet{ning-etal-2018-joint, do-etal-2011-minimally}.} where each tail event is presented with all preceding events. The annotator needs to determine \emph{why the tail event has happened} and then verify if the causing event is among the listed candidates. This in contrast to the RED \cite{ogorman-etal-2016-richer} annotation methodology, where given an event pair, involves assessing if \emph{the tail event is inevitable given the head event}. We further discuses our motivation for adopting the EventStoryLine methodology in §\ref{tool:logic}.

%The coreference and causal relations are constrained by the temporal relation. Event mentions that corefer must be identical in time and duration. For an event to cause another, it must start \emph{before} the affected event.


% \subsection{Completeness and Consistency}
% \label{back:compl-consist-complex}


%by identifying all pairs of events that require annotation and preventing contradictions in direct, transitive, and across different types of relations (for example, a \emph{cause} must align with a \emph{before} temporal relation). (2) Reducing annotation \emph{complexity} to make the process feasible and manageable for annotators.

% To that end \App{} is integrated with a framework that enforce these attributes, as further detailed in §\ref{tool:logic}.

\subsection{Existing Annotation Tools}
\label{back:annot-tools}

%Existing datasets that encompass the temporal, coreference and causal relations (or a subset of these relations) \cite{chaturvedi-etal-2017-story, mirza-etal-2014-annotating, hong-etal-2016-building, ogorman-etal-2016-richer, wang-etal-2022-maven}, have either utilized and customized general-purpose tools such as BRAT \cite{stenetorp-etal-2012-brat} or CAT \cite{bartalesi-lenzi-etal-2012-cat}, or did not release or specify the use of any annotation tool.

%Currently, to establish multiple event-event relation annotation, two options are available: (1) using general-purpose annotation tools like BRAT \cite{stenetorp-etal-2012-brat} and CAT \cite{bartalesi-lenzi-etal-2012-cat}, which offer extensive customization and administrative capabilities. 
%However, they lack specific implementations crucial for managing the complexity of event relation annotations by ensuring completeness and consistency. (2) using multiple event annotation tools, each dedicated to a specific relation type. Yet, all temporal annotation tools \cite{cassidy-etal-2014-annotation, derczynski-etal-2016-gate, fulda-etal-2016, rogers2022narrativetime} follow the TimeML annotation scheme, while no existing tool that we know of supports causal annotation. Furthermore, using multiple tools to annotate different types of relations presents significant challenges in terms of management and maintenance. To address these issues, we developed \App{} to meet specific needs of event relation annotation within a single unified workflow.

% Currently, There are two primary methods for annotating multiple event-event relations. One method involves adapting \textit{general-purpose} annotation tools like BRAT \cite{stenetorp-etal-2012-brat} and CAT \cite{bartalesi-lenzi-etal-2012-cat} for constructing relation graphs. 
% However, these tools lack specific features for addressing the specific needs of event relation annotations, such as ensuring completeness, consistency, and leveraging the characteristics of such graphs to manage complexity. 
% The other method involves using multiple dedicated tools, each for a specific type of relation. 
% Yet, existing annotation tools for temoral relations \cite{cassidy-etal-2014-annotation, derczynski-etal-2016-gate, fulda-etal-2016, rogers2022narrativetime} adhere to the TimeML annotation scheme, and none support causal relations annotation.
% Additionally, using multiple tools poses challenges in terms of management and maintenance. 
% To address these issues, we develop \App{}, designed specifically for annotating multiple event-event relations within a unified workflow.

Currently, there are two primary methods for annotating multiple event-event relations. One involves adapting \textit{general-purpose} annotation tools like BRAT \cite{stenetorp-etal-2012-brat} and CAT \cite{bartalesi-lenzi-etal-2012-cat}. However, these tools lack features for event relation annotations, such as ensuring completeness, consistency, and managing annotation complexity. The other method involves using multiple dedicated tools for specific relations. Yet, existing tools for temporal relations \cite{cassidy-etal-2014-annotation, derczynski-etal-2016-gate, fulda-etal-2016, rogers2022narrativetime} follow the TimeML annotation scheme, and none support causal relations annotation. 
Additionally, the use of multiple tools introduces further challenges. To address these issues, we developed \App{} to annotate multiple event-event relations in a single unified workflow.


%%%%%%%%%%%%%%%%%%% START PREVIOUS VERSION %%%%%%%%%%%%%%%%%%%
% Currently, there are two main approaches to annotating multiple event-event relations: (1) using general-purpose annotation tools like BRAT \cite{stenetorp-etal-2012-brat} and CAT \cite{bartalesi-lenzi-etal-2012-cat}, adapted for relation graphs. However, these tools lack specific features crucial for managing the complexity of event relation annotations, such as ensuring completeness, consistency, and effectively handling complexity. (2) employing multiple dedicated tools, each for a specific type of relation. Yet, all known temporal annotation tools \cite{cassidy-etal-2014-annotation, derczynski-etal-2016-gate, fulda-etal-2016, rogers2022narrativetime} adhere to the less-efficient TimeML annotation scheme, and there are no existing tools that support causal annotation to our knowledge. Furthermore, using multiple tools poses significant challenges in terms of management and maintenance. In response to this gap, we developed \App{} to specifically cater to the needs of multiple event-event relations annotation within a single unified workflow.
%%%%%%%%%%%%%%%%%%%% END PREVIOUS VERSION %%%%%%%%%%%%%%%%%%%%%%


% To the best of our knowledge, \App{} is the first annotation tool to support end-to-end annotation of temporal, causal, and coreference relations, enforcing completeness and consistency while managing complexity (further detailed in §\ref{tool}).

% In the individual relation annotation space, a variety of tools have been developed over the years for specific tasks, such as temporal relation annotation \cite{verhagen-etal-2006-annotation, verhagen-pustejovsky-2008-temporal, cassidy-etal-2014-annotation, derczynski-etal-2016-gate, fulda-etal-2016, rogers2022narrativetime}, and coreference \cite{girardi-etal-2014-cromer, oberle-2018-sacr, bornstein-etal-2020-corefi}.\footnote{To the best of our knowledge, no tool exists specifically for annotating causal relations.} However, most temporal annotation tools adhere to the TimeML scheme. Additionally, using multiple tools to annotate different types of relations poses significant challenges in terms of handling and maintenance.



==> emnlp_sec/intro.tex <==
\section{Introduction}
\label{intro}
%Understanding events and their relations is crucial in natural language understanding (NLU) \cite{ MillerJohnsonLaird+1976, levelt-etal-1993}. 
Events and their relations are often illustrated as graphs, with nodes representing events and edges denoting inter-event relations, such as temporal \cite{do-etal-2012-joint} and causal \cite{chaturvedi-etal-2017-story}. Such graphs are pivotal in various applications like detecting misinformation \cite{lei-huang-2023-identifying} and biases \cite{lei-huang-2024-sentence}, common-sense reasoning \cite{gao-etal-2023-chatgpt, chan-etal-2024-exploring}, and question-answering \cite{10083216}.

% Events and the relations between them are often depicted as graphs, where nodes represent events \cite{raghunathan-etal-2010-multi}, and edges indicate various relations such as temporal \cite{do-etal-2012-joint} and causal \cite{chaturvedi-etal-2017-story}. Event relation graphs are pivotal in various applications such as detecting misinformation \cite{lei-huang-2023-identifying} and biases \cite{lei-huang-2024-sentence}, common-sense reasoning \cite{gao-etal-2023-chatgpt, chan-etal-2024-exploring}, and question-answering \cite{10083216}.

However, high-quality, densely annotated event relation graphs are rare due to the linguistic complexity involved in identifying these relations, as reflected by low Inter-Annotator Agreement (IAA) in current datasets \cite{hong-etal-2016-building, ogorman-etal-2016-richer}. Additionally, annotating relations between \textit{all} event pairs for each relation type is impractical for large sets of events, leading some studies to focus only on relations between consecutive sentences \cite{chambers-etal-2014-dense, ning-etal-2018-joint}.
Moreover, commonly used annotation tools \cite{stenetorp-etal-2012-brat, bartalesi-lenzi-etal-2012-cat} are general-purpose and fail to meet the specific needs of event relation graph annotation, such as managing complexity and addressing contradictory or incomplete annotations.


%characteristics and needs of event relation graphs. These include utilizing transitive closure algorithms to manage complexity and handling issues like contradictory relations and incomplete annotations.


% Despite their importance, high-quality and densely annotated datasets of event relation graphs are scarce. The main reason is the linguistic complexity of identifying these relations, as evidenced by the low Inter-Annotator Agreement (IAA) reported in existing datasets \cite{hong-etal-2016-building, ogorman-etal-2016-richer}. Additionally, the process involves the need to evaluate relations between all event pairs, making exhaustive annotation impractical for large sets of events. To address this, some studies have limited annotations to relations between consecutive sentences only \cite{chambers-etal-2014-dense, ning-etal-2018-joint}. Moreover, commonly used annotation tools such as \cite{stenetorp-etal-2012-brat, bartalesi-lenzi-etal-2012-cat} are general-purpose and do not leverage the specific characteristics of such relations, like employing transitive closure algorithms to reduce complexity, preventing contradicting relation, or addressing incomplete annotations. Consequently, exhaustively annotated resources that cover relations across entire documents remains a challenge.





% \avivs{Is there a way to use some example to exemplify the aforementioned challenges?}

\begin{figure*}[t!]
\centering
\includegraphics[width=\textwidth]{latex/figures/figure1.png}
\caption{\App{} annotation steps: [1] Event Selection: Annotators select events that are ``anchorable'' in time. [2] Temporal Relations Annotation: Annotators establish temporal relations between pairs of event mentions. [3] Coreference Annotation: Annotators identify co-occurring event mentions. [4] Causal Annotation: Annotators determine whether a causal relation exists between events.}
\label{fig:figure1}
\end{figure*}
%\caption{An illustration of \App{} steps: (1) Actual event selection; (2) Temporal relation annotation; (3) Coreference relation annotation; (4) Causal relation annotation.}

To bridge this gap, we introduce \App{}, a novel tool designed for \textit{complete}, high-quality annotation of temporal, coreference, and causal event relations within a single unified workflow (§\ref{back:compl-consist-complex}). We simplify this complex task by segmenting it into four manageable steps, illustrated in Figure~\ref{fig:figure1}. Each step builds upon the previous, utilizing well-established schemes and algorithms (§\ref{back:annot-schemes}) to ensure comprehensive, high-quality annotations with reduced complexity.

To address the impracticality of \textit{exhaustively} annotating all events, the first step in \App{} involves annotators identifying significant events in the story (§\ref{tool:event-select}), thereby narrowing the scope of annotation and making exhaustive annotation feasible across the entire document. Subsequent steps streamline the annotation of all three relation types. Starting with temporal relations (§\ref{tool:temp}), \App{} uses a transitive closure algorithm to infer and auto-annotate transitive relations, thereby reducing workload. These temporal annotations then help refine the scope for the subsequent coreference annotation step (§\ref{tool:coref}) by focusing only on co-occurring events. In the final step, causal relation annotation, \App{} considers only preceding events and uses coreference annotations to treat coreferring mentions as a single event, to avoid redundant annotations.
% To bridge this gap, we present \App{}, a novel tool for \textit{complete}, high-quality annotation of temporal, coreference, and causal event relations within a single unified workflow (§\ref{back:compl-consist-complex}). We simplify this complex task by breaking it into four manageable steps, as illustrated in Figure~\ref{fig:figure1}. Each step builds on annotations from previous steps and employs well-established schemes and algorithms (§\ref{back:annot-schemes}) to ensure \textit{complete}, high-quality annotations with reduced complexity.
% To address the impracticality of \textit{exhaustively} annotating all events, the first step in \App{} focuses on narrowing the scope of annotation to only significant events (§\ref{tool:event-select}), making the annotation process more manageable.
% The following steps are intended at streamlining the \textit{exhaustive} annotation of all three relation types, starting with temporal relations (§\ref{tool:temp}), \App{} employs a transitive closure algorithm to infer and auto-annotate transitive relations to reduce workload. These temporal annotations subsequently aid in refining the scope for coreference annotations (§\ref{tool:coref}) by focusing only on co-occurring events. Finally, in causal relation annotation, \App{} also leverages previous coreference annotations to treat coreferring mentions as a single event, thus minimizing redundant annotations.
%Initially, annotators identify significant events in the story (§\ref{tool:event-select}), thereby narrowing the scope of annotation and making \textit{exhaustive} relation annotation across the entire document more manageable. 
%The following steps are intended at streamlining the \textit{exhaustive} annotation of all three relation types, starting with temporal relations, then coreference, and concluding with causal relations, focusing on one relation type at a time. 
%The following steps then streamline the annotation of all three relation types, starting with temporal relations, then coreference, and concluding with causal relations, focusing on one relation type at a time. 
%For temporal annotations (§\ref{tool:temp}), \App{} employs a transitive closure algorithm to infer and auto-annotate transitive relations, reducing the overall workload. 
%\App{} then uses these temporal relations to selectively present relevant pairs for annotation in subsequent steps: co-occurring pairs for coreference (§\ref{tool:coref}) and preceding pairs for causal relations (§\ref{tool:cause}). In causal relation annotation, \App{} also leverages previous coreference annotations to treat coreferring mentions as a single event, thus minimizing redundant annotations.
%These temporal annotations subsequently aid in refining the scope for coreference annotations (§\ref{tool:coref}) by focusing only on co-occurring events. Similarly, for causal relations (§\ref{tool:cause}), \App{} considers only preceding events and uses coreference annotations to treat coreferring mentions as a single event, to avoid redundant annotations.
Furthermore, to ensure consistency and completeness, \App{} detects and alerts annotators to any inconsistencies or missing relations throughout the process.

% The subsequent steps are designed to streamline the exhaustive annotation of the aforementioned three types of relations, with annotators focusing on one event at a time. The process begins with temporal relation annotation, followed by coreference, and concludes with causal relations. For temporal relations  (§\ref{tool:temp}), \App{} employs a transitive closure algorithm to infer and auto-annotate transitive relations, thus reducing the overall workload. 
% These temporal annotations are then leveraged to further narrow the annotation scope of coreference relations (§\ref{tool:coref}), by only focusing on co-occurring events. Likewise, for the causal relations (§\ref{tool:cause}), \App{} only focuses on preceding events, while also leveraging the coreference relations to treat coreferring event mentions as a single event, thereby avoiding redundant annotations.
% Additionally, \App{} actively identifies and alerts annotators to any contradictions or missing relations, ensuring high-quality annotations.




%To that end, following \cite{ning-etal-2018-multi} we consider events that actually occurred or will occur, filtering intentional or hypothetical events (§\ref{tool:event-select}).
%This makes the exhaustive annotation of event relation across the entire document feasible.
% we adopt the Multi-Axis methodology of \cite{ning-etal-2018-multi} and restrict the number of events within a document to only those that actually occurred or will occur, in contrast to intentional or hypothetical events (§\ref{tool:event-select}).
%(``anchored in time'').
%The first two steps of the annotation procedure adopt the Multi-Axis methodology \cite{ning-etal-2018-multi}. The initial step narrows the scope of the annotation to This approach is motivated by the understanding that establishing relations between actual and non-actual (i.e., intentional or hypothetical) events is impractical, thus focusing the annotation scope solely on actual events (§\ref{tool:event-select}). 
% The subsequent steps focus on streamlining the exhaustive annotation of the three aforementioned relations. Starting with temporal, followed by coreference, and concluding with causal. For temporal relation annotation (§\ref{tool:temp}), \App{} uses a transitive closure algorithm to infer and automatically annotate transitive relations after each step. These temporal annotations are then leveraged in the coreference annotation step (§\ref{tool:coref}), focusing on co-occurring event pairs. For the causal relation annotation (§\ref{tool:cause}), \App{} utilizes both temporal and coreference annotations to reduce complexity. Additionally, to ensure high annotation quality, \App{} actively detects and alerts on any contradicting or missing relations.

%To manage complexity, for temporal (§\ref{tool:temp}) and coreference (§\ref{tool:coref}) relations, \App{} uses a transitive closure algorithm to infer and auto-annotate transitive relations following each annotation step. Additionally, for the coreference relation, \App{} leverages temporal annotations from the previous step to focus only on co-occurring event pairs. For causal relations (§\ref{tool:cause}), \App{} utilizes both temporal and coreference relations to reduce complexity. Furthermore, \App{} adopts the EventStoryLine methodology \cite{caselli-vossen-2017-event} for causal annotation, which has proven in our experiments to be more intuitive than other annotation paradigms.
%Finally, to ensure high annotation quality, \App{} also detects and alerts annotators to any contradicting relations.

To evaluate \App{}, we conduct a pilot study to assess the annotation complexity and quality (§\ref{pilot}). Our findings indicate that our tool significantly simplifies the annotation process, reducing the complexity of temporal, coreference, and causal annotations by 56\%, 96\%, and 41\% respectively. \App{} also leads to high-quality annotations, as evidenced by strong inter-annotator agreement. The tool and code are publicly available at \url{https://github.com/AlonEirew/EventGraphAnnot}.

% Overall, \App{} streamlines the complex annotation process of event relations, ensuring consistency and completeness in a unified framework for annotating temporal, coreference, and causal relations.

==> emnlp_sec/pilot.tex <==
\section{Pilot Study}
\label{pilot}

To evaluate \App{}'s effectiveness, we run a small-scale study to assess two aspects:
(1) the time and effort needed to complete the annotation, and (2) the quality of the annotated relation graphs through Inter-Annotator Agreement (IAA). 
This section details the annotation procedure (§\ref{pilot:annot-proc}) and reviews the quality and effectiveness of the annotation process (§\ref{pilot:results}).

%involving three non-expert annotators who received training for each task. This trial 
%We evaluated the annotation we considered two aspects of the annotation: (1) We selected 6 documents from the TCR  dataset. Within each document, 10 gold mentions were chosen according to the following criteria: events participating in causal relationships were given priority 

%from each document we  which the annotators then annotated end-to-end using \App{}. 

\subsection{Annotation Procedure}
\label{pilot:annot-proc}
For the user study, we hire three non-expert annotators, all native English speakers and either first-degree students or graduates. They first undergo 2-3 training iterations on each sub-task using 2-3 test documents to ensure adequate understanding of the tasks.
The actual annotation is performed over six news documents, each around 500 words. We use the model from \citet{cattan-etal-2021-cross-document} to identify event-mention candidates, and GPT-4 \cite{achiam2023gpt} to extract temporal entities.

% At first, annotators were provided with the annotated documents along with the \App{} tool, and was tasked with the initial step of selecting event mentions that are anchorable in time (§\ref{tool:event-select}. Following this, one of the paper's authors reviewed the event mentions in each document and selected 15-18 mentions from each that are significant to the underlying story.

Annotators first identify ``anchorable'' event mentions (§\ref{tool:event-select}), limited to no more than 20 per document, followed by the annotation of the three event relation types.
For temporal relations, annotators are instructed to first read the article and annotate the most obvious temporal relations by clicking on the relevant edges in the accompanying graph visualization. This approach has proven effective in helping them better understand the underlying story and avoid simple mistakes. 
Since this initial pass usually yields only a few annotations, they then make a second pass to address the remaining pairs.
For coreference and causal relations, annotators are instructed to use the ``Next Unhandled'' button to progress through the annotations.
At any point, Annotators can revise annotations as needed using the navigation buttons (available in all steps) or the graph visualization (editable only in the temporal step).
Finally, we measure Inter-Annotator Agreement (IAA), annotation time, and the number of annotation steps for each phase.



% Annotators first identify \textit{anchorable} event mentions (§\ref{tool:event-select}), limited to no more than 18 per document to manage the study’s scope, followed by the annotation of the three event relation types.
% For temporal relations, annotators are instructed to first read the article and annotate clear temporal relations, by clicking on the relevant edges in the accompanying graph visualization. 
% We found that this approach helped them get a better understanding of the underlying story as well as avoid simple mistakes. Upon annotating the entire document once, annotators make a second pass to attend to the unannotated pairs, via the ``Next Unhandled Pair''. 
% For coreference and causal relations, they are instructed to only use the ``Next Unhandled Event'' button for navigation. 
% At any point, annotators can use the navigation buttons to revise earlier annotations as needed.
% Finally, we measure Inter-Annotator Agreement (IAA), annotation time, and number of annotation steps for each step.

%%%%%%%%%%%%%%%%%%% START PREVIOUS VERSION %%%%%%%%%%%%%%%%%%%
% Annotators first identify the \textit{anchorable} event mentions (§\ref{tool:event-select}), limited to no more than 18 mentions per document for the purposes of the user study.
% Next, they proceed with the annotation of the three event relation types. For temporal relations, we instruct them to first read the article carefully, and whenever coming across event mention pairs whose temporal relation is easily understood, to annotate them using the tool's graph visualization feature, by clicking the relevant edge and annotating it.
% We found that this approach helps annotators get a better understanding of the underlying story and later avoid simple errors. Upon completing one pass over the document, they are asked to make a second pass, beginning with the first unannotated pair in the document and following the tool's suggestions via the `Next Unhandled Pair'' button. For coreference and causal annotations, annotators are instructed to use only the Next Unhandled Event'' button for navigation. At any stage, they can modify previous annotations as needed, via the navigation buttons.
% Finally, we measure the Inter-Annotator Agreement (IAA), annotation time, and number of annotation steps for each individual step.
%%%%%%%%%%%%%%%%%%%%%% END PREVIOUS VERSION %%%%%%%%%%%%%%%%%%



%Subsequently, one of the paper's authors reviewed the event mentions in each document and selected 15-18 mentions from each to further reduce annotation scope.
%For the annotation process we selected six news documents, each containing an average of 500 words. As a preliminary step, we used the model from \cite{cattan-etal-2021-cross-document} to extract event candidates from each document. Subsequently, each annotators were given the six document along with \App{} and was tasked with the initial step of assigning events to their correct axis (§\ref{tool:annot-flow} step 1). Following this, one of the authors reviewed the events and selected from each document 13-18 events that are on the main axis and most relevant to the underlying story.


%\cite{fabbri-etal-2019-multi} corpus. The motivation for selecting this resource is that the CNN summaries nicely cover the unfolding of major events and are considered challenging news articles (\alone{find citation for last sent or remove}). We selected summaries that cover at least five articles, each with an average of 500 words per summary.

% For the temporal annotation, we spitted the 15 documents to three groups each with 5 documents. Each group was assign to two different annotators which separately conducted the temporal relation annotation (§\ref{tool:annot-flow} step 2). Following this step we measure the IAA, time and number of annotation steps (presented next in §\ref{pilot:results}) for the temporal relation annotation task.

%For the temporal annotation, we divided the 15 documents into three groups, each consisting of 5 documents. Each group was assigned to two different annotators who independently conducted the temporal relation annotation (§\ref{tool:annot-flow} step 2). We instructed the annotators to first read the entire article without making any annotations. Then, during the second pass, they were to use the graph visualization tool (§\ref{tool:feat}) to annotate pairs between which they had already identified the relation. Finally, we asked the annotators to proceed by using the "Next Unhandled Pair" feature to annotate the remaining pairs.

%Following this step, we measured the Inter-Annotator Agreement (IAA), time, and number of annotation steps for the temporal relation task.

%Next, each group of documents was assigned to the third annotator who had not previously worked on that group. This annotator's role was to adjudicate all relations on which the first two annotators disagreed. This consolidation step is crucial for dense annotation, as subsequent steps are constrained by the temporal relations established here—\emph{equal} for coreference and \emph{before/after} for causal relations (§\ref{tool:annot-flow} step 3). This step ensures that in the next steps, annotators are presented with (1) all relevant temporal relations, and (2) a unified set of candidates.

%After the consolidation step, for the final two steps—coreference and causal relations annotation—all three annotators were given the same five sampled documents to annotate. We then measured the Inter-Annotator Agreement (IAA), time, and number of annotation steps for this task. 
%The results are presented in the following section §\ref{pilot:results} and in Table~\alone{ref to table}.

\input{latex/tables/agree_tab}

\subsection{Analysis}
\label{pilot:results}
% \avivs{Should use better discourse, e.g., "We first note that..."} 
We first note that agreement between annotators, as shown in Table~\ref{tab:annot_agree}, is notably high for all three relations, indicating that our annotation tool effectively assists in generating high-quality annotations, without compromising completeness and consistency. 
We also observe in Table~\ref{tab:annot_time} that the annotation of temporal relations roughly takes 44.3 minutes to complete, which is significantly more demanding than the other two types of relations. 
%the latter two relations benefit from the temporal relation annotation to further reduce the overall workload.
This finding is sensible, given that temporal relation annotation requires making one of four possible decisions (e.g., before, after, equal, uncertain) for each pair of events. In contrast, coreference and causal relations involve identifying connections within a set of events relative to a focal event. 
Importantly, Table~\ref{tab:annot_step} indicates that \App{} assists in significantly reducing complexity for all three relation types.
\\~\\
Overall, our annotation process generates complete and consistent graphs covering temporal, causal and coreference relations while maintaining simplicity. 
The use of transitive closure algorithms reduced the manual workload for temporal relation annotation by 56\% and prevented inconsistency errors, along with the discrepancy identification algorithm.
Our decision to use the EventStoryLine approach over the RED approach for causal relation annotation, based on preliminary analyses showing higher annotator agreement with the former,\footnote{See Appendix~\ref{app:cause-scheme-expr}.} has also proven effective.
Finally, the task order also helped in streamlining the annotation process. Beginning with temporal relation annotation allowed subsequent steps to focus only on the relevant subset of pairs, leveraging the time constraint between temporal and other relations. This was particularly effective for coreference annotation, where the workload was reduced by 96\% (see Table~\ref{tab:annot_step}). Additionally, annotating coreference before causal relations enabled us to treat coreferring event mentions as single events, further reducing redundancy.


%%%%%%%%%%%%%%%%%%% START PREVIOUS VERSION %%%%%%%%%%%%%%%%%%%
% We first note that agreement between the annotators, as presented in Tables~\ref{tab:annot_agree}, is notably high across these tasks, indicating that our annotation tool effectively assists in generating high-quality annotations, while also ensuring completeness and consistency.
% From Table~\ref{tab:annot_time}, it is evident that annotating temporal relations is the most time-consuming task, requiring each annotator an average of 44.3 minutes to complete one document, while causal relations require 17.3 minutes, and coreference - 7.7 minutes. Table~\ref{tab:annot_step} indicates that \App{} assists in reducing complexity for temporal annotations by an average of 56\%, making the task feasible at this scale, and for causal annotations by 41\%. This reduction in causal annotation, combined with the EventStoryLine annotation scheme \cite{caselli-vossen-2017-event}, significantly expedites and simplifies the annotation process.
% \\~\\
% Overall, our annotation process produces complete and consistent graphs covering temporal, causal and coreference relations while maintaining simplicity. Using transitive closure algorithms significantly reduced the manual workload in temporal relation annotation by 56\%. This algorithm also help in preventing inconsistency errors in the generated data.
% Additionally, we choose the EventStoryLine approach for causal relation annotation after finding it superior to the RED approach in terms of inter-annotator agreement, indicating greater efficiency and simplicity (our experiments with both schemes are further detailed in Appendix~\ref{app:cause-scheme-expr}). 
% Finally, the task order further streamlined the process. Beginning with temporal relation annotation allowed subsequent steps to focus only on the relevant subset of pairs, leveraging the time constraint between temporal and other relations. This was particularly effective for coreference annotation, where the workload was reduced by 95\%. Additionally, annotating coreference before causal relations enabled us to treat coreferring event mentions as single events, further reducing redundant and preventing inconsistent annotations.
%%%%%%%%%%%%%%%%%%%%%% END PREVIOUS VERSION %%%%%%%%%%%%%%%%%%

%For coreference and causal annotations, coreference tasks are typically completed quickly due to the smaller number of relations needed for annotation. In contrast, causal annotations involve a much larger set of relations (as discussed in §\ref{tool:annot-flow}). While our tool achieves a 20\% reduction in complexity, the EventStoryLine annotation scheme \cite{caselli-vossen-2017-event} significantly simplifies this task.

%Finally, we observed disparity in performance among annotators. For instance, while annotator B completed the task in 76 minutes, annotator C took 111 minutes and made more temporal annotation steps, also showing lower agreement with others. This indicates that C struggled more with decision-making and may require additional training.

%For temporal annotation, annotators considered, on average, 15.2 mentions per document, totaling 228 mentions. The complete temporal graph would have required each annotator to annotate 1,635 pairs; however, less than 40\% of these relations required actual annotation to receive the complete graph. This indicates that the transitive closure and annotation flow significantly reduce the annotation complexity. Overall, annotators spent an average of 45 minutes annotating each document for temporal relations, and achieved 0.72 Cohen Kappa agreement, which is considered to be high agreement for this task.

%unlike the RED approach, it is inherently non-transitive,\footnote{The justification for this can be further explored in the original paper} thus avoids inconsistency risks.

==> emnlp_sec/tool.tex <==
\section{The \App{} Annotation Tool}
\label{tool}
\App{} is a web-based tool designed to facilitate the annotation of \textit{complete} and \textit{consistent} event relation graphs over a manageable subset of temporally anchorable events, covering temporal, coreference, and causal relations (illustrated in Figure~\ref{fig:figure1}).
It takes as input a document with pre-identified event mentions, obtained using any off-the-shelf event extraction model, as well as an optional set of extracted temporal entities, highlighted in the text to aid the annotation process.
The tool employs a layered annotation approach over the provided set of events, breaking the annotation process into four smaller, more manageable sub-tasks: event selection (§\ref{tool:event-select}), temporal relations annotation (§\ref{tool:temp}), coreference annotation (§\ref{tool:coref}), and causal relations annotation (§\ref{tool:cause}) (see screenprints of \App{} in Appendix~\ref{appx:additional_printscreens}).

%%%%%%%%%%%%%%%%%%% START PREVIOUS VERSION %%%%%%%%%%%%%%%%%%%
% \App{} is a web-based tool designed to facilitate the annotation of complete event relation graphs, encompassing temporal, coreference, and causal relations (illustrated in Figure~\ref{fig:figure1}).
% Since our tool was not designed for event detection annotation, documents should have the initial set of event mentions extracted using any off-the-shelf event extraction model. Optionally, temporal entities can also be extracted, allowing \App{} to highlight them in the text.

% \App{} employs a layered annotation approach that decomposes the annotation process into four smaller, more manageable sub-tasks: event selection (§\ref{tool:event-select}), temporal relations annotation (§\ref{tool:temp}), coreference annotation (§\ref{tool:coref}), and causal relations annotation (§\ref{tool:cause}).
%%%%%%%%%%%%%%%%%%%%%% END PREVIOUS VERSION %%%%%%%%%%%%%%%%%%


% Facilitating the annotation of a complete event-event relation graph, including temporal, coreference, and causal relations, is challenging. First, we selected annotation schemes that ensure two key attributes: support exhaustive annotation between all events, and simplify the annotation to increase agreement (§\ref{back:annot-schemes}).

% However, to make annotation feasible, it is essential to manage the quadratic annotation complexity of each relation type while ensuring the resource is complete and consistent (§\ref{back:compl-consist-complex}). 
% Given the high number of pairs requiring consideration for each relation type, it is unrealistic to expect annotators to adhere perfectly to these three constraints. To accomplish this, \App{} provides a supportive framework that aids annotators in their tasks. This framework leverages the two levels of granularity required for this type of annotation: (1) across the different tasks, and (2) within each specific required annotation task.

% by instructions (adheres to the annotation guidelines described in §\ref{back:annot-schemes}), and provided with the document text, the highlighted events to consider and a straightforward questions that annotators are required to answer. 


% Starting the relation annotation with the temporal task is strategic, as it allows for leveraging the temporal constraints (as detailed in §\ref{back:event-rels}) in subsequent coreference and causal annotation steps.
% For the succeeding coreference task, 
% annotators are presented only with candidate pairs previously annotated with an \emph{equal} temporal relation. This approach is based on our observations and those reported in prior work \cite{ogorman-etal-2016-richer, wang-etal-2022-maven, rogers2022narrativetime}, where \emph{equal} relations constitute about 5\% of all relations. Thus, considering only event mentions with an \emph{equal} relation dramatically reduces the annotation complexity in this step.



\subsection{Event Selection}
\label{tool:event-select}
% The first step aims to narrow the annotation scope by choosing only event mentions that can be anchored in time ((1) in Figure~\ref{fig:figure1}).
% Following the Multi-Axis methodology \cite{ning-etal-2018-multi}, annotators review a document with highlighted event mentions, identifying those that are ``anchorable in time'' (§\ref{back:annot-schemes}).
% Only these ``anchorable'' events are then considered in subsequent steps, making the exhaustive annotation of event relations across the entire document more manageable.

% The first step aims to narrow the annotation scope by selecting only event mentions that can be anchored in time ((1) in Figure~\ref{fig:figure1}). Following the Multi-Axis methodology \cite{ning-etal-2018-multi}, annotators review a document with highlighted event mentions and identify those that are ``anchorable in time'' (§\ref{back:annot-schemes}). Only these anchorable events are considered in subsequent steps, making the exhaustive annotation of event relations across the entire document more manageable.

The first step aims to narrow the annotation scope by selecting only event mentions that can be anchored in time ([1] in Figure~\ref{fig:figure1}). Following the Multi-Axis methodology \cite{ning-etal-2018-multi}, annotators review a document with highlighted event mentions and identify those that are ``anchorable in time'' (§\ref{back:annot-schemes}). Only these anchorable events are considered in subsequent steps, making the exhaustive annotation of event relations across the entire document more manageable.


\alone{In large documents, however, temporal annotation remains challenging (as further discussed in our analysis \ref{pilot:results}), making it necessary to further narrow the set of event mentions. To address this, we instruct annotators to limit the event mention set to the 20\footnote{Beyond this, annotation becomes less manageable.} most significant events in the story.\footnote{While there is no precise scientific measure of event significance, a downstream task can define what is significant for its specific use case.} This annotation approach differs from current methods; instead of selecting specific edges to annotate across all mentions, our approach considers all relations between a selected subset of events. Annotating all relations between all event mentions in large documents remains a challenge for future research.}



% and from these filter out the most significant events\footnote{Though there is no scientific measure of event significancy, a downstream task can determine what is significant for it}. This narrowing to consider only significant event mentions is required in long documents as annotating a large set of events remains a challenge.

% The initial phase focuses on selecting the most critical events in the text ((1) of Figure~\ref{fig
% }). Utilizing the Multi-Axis methodology \cite{ning-etal-2018-multi}, annotators review a document with highlighted event mentions,\footnote{For event detection, we use the model from \cite{cattan-etal-2021-cross-document}.} identifying those that are "anchorable in time" (§\ref{back
% }). Only these "anchorable" events are considered in subsequent steps, streamlining the comprehensive annotation of event relationships across the document.


% The initial step in the annotation process focuses on reducing the annotation scope by selecting only the most significant events in the story ((1) of Figure~\ref{fig:figure1}). Inspired by the Multi-Axis methodology \cite{ning-etal-2018-multi}, annotators are presented with a document highlighted with event mentions. They are tasked with identifying the actual (``anchorable'' in time) or non-actual events (§\ref{back:annot-schemes}). 
%To further eliminate non-significant events, annotators are asked to remove reporting events (e.g., John from CNN \textit{\underline{reported}}) which do not contribute to the narrative.
% Then, only events labeled as ``anchorable'' are considered in subsequent steps. This step makes the exhaustive annotation of event relations across the entire document more manageable.

%The initial step in the annotation process focuses on reducing the annotation scope by selecting only the most significant events in the story (Step 1 of Figure~\ref{fig:figure1} and Figure~\ref{fig-appx:select}). Inspired by the Multi-Axis methodology \cite{ning-etal-2018-multi}, annotators are presented with a document in which event mentions have been extracted\footnote{Using \cite{cattan-etal-2021-cross-document} event detection model.} and are now highlighted, and are tasked with identifying the actual (``anchorable'' in time) or non-actual events. Then, only events labeled as ``anchorable'' are considered in subsequent steps. 
%It is worth noting that in long documents, the number of actual events can be high making the annotation still time consuming, in such cases, 

% or if it did not actually happen (e.g., events that are intentional, hypothetical, recurring, etc.).

\subsection{Temporal Relation Annotation}
\label{tool:temp}
% The next step involves \emph{temporal} relation annotation (Step 2 of Figure~\ref{fig:figure1} and Figure~\ref{fig-appx:temporal}). Here, annotators are presented with one pair of event mentions at a time and are tasked with deciding which one started first, or whether they started at the same time. Importantly, to ensure \textit{exhaustiveness}, this step cannot be completed until all event mention pairs have been annotated. However, iterating through all pairs in a single document is a very time-consuming and challenging task. Therefore, to reduce \textit{complexity}, a transitive closure algorithm identifies and automatically annotates non-annotated pairs, thereby alleviating the need for their manual annotation.\footnote{For more details, see §\ref{appx:transitive-constraints}.}
% Finally, to ensure \textit{consistency}, an inconsistency-detection algorithm runs in the background to alert annotators of discrepancies, such as event A annotated before event B, event B before event C, and event C before event A.\footnote{For more details, see §\ref{appx:discrepancy}.}

The next step involves annotating \emph{temporal} relations ([2] in Figure~\ref{fig:figure1}), with the goal of establishing links between \textit{all} pairs of ``anchorable'' event mentions. Annotators review these pairs within their context, presented one at a time, where one event is marked in red and the other in green. Temporal entities, if extracted, are also highlighted. Alongside this, a visualization of the updating relation graph is provided, with the scrutinized pair emphasized. Annotators must determine whether one of the events started first, if both started simultaneously, or if the timeline is uncertain. Notably, the graph visualization aids in tracking progress and enhances flexibility, allowing annotators to directly select and annotate (or fix) pairs by clicking on the corresponding graph nodes.
%\footnote{The ``Next'' and ``Back'' buttons scroll through the pairs, and ``Next Task'' and ``Prev Task'' buttons scroll through the different annotation tasks.} 


% The next step involves annotating \emph{temporal} relations ((2) in Figure~\ref{fig:figure1}), aiming to establish links between \textit{all} pairs of ``anchorable'' event mentions.
% Annotators review these pairs within their context, marked in red and blue (as shown in Figure~\ref{fig:figure1}),\footnote{Temporal entities, if extracted, are also marked.} alongside a visualization of the updating relation graph, with the scrutinized pair highlighted.
% Annotators need to decide if an event precedes another, both start concurrently, or the timeline is uncertain.
% Notably, in addition to helping track progress, the graph visualization also provides flexibility, allowing annotators to directly select and annotate (or fix) pairs by clicking on the corresponding graph nodes, on top of using the navigation buttons.


% The next step involves \emph{temporal} relation annotation ((2) in Figure~\ref{fig:figure1}), where the goal is to establish a temporal relation between all pairs of the ``anchorable'' event mentions. Annotators are presented with a pair of event mentions within the context, one event marked in red and the other in blue (as shown in Figure~\ref{fig:figure1}),\footnote{If temporal entities were extracted, they are also marked.} along with a graph visualization of the current annotation state highlighting the pair. Annotators are asked to determine whether one of the events started first, if both started simultaneously, or if the timeline is uncertain.

\input{latex/tables/disc_temp}

%To improve the annotation phase, we modified the original Multi-Axis format, which involved two binary questions per relation (detailed in §\ref{back:annot-schemes}). This format was found to be non-intuitive and added unnecessary complexity. To streamline the process, we revised the method, allowing annotators to directly 

To ensure the desirable graph traits of completeness and consistency (§\ref{back:compl-consist-complex}), this step can only be completed when all pairs of event mentions have been annotated without any contradicting relations. Given the extensive number of pairs, expecting annotators to perfectly comply with these standards is unrealistic.

To address this challenge, \App{} employs a transitive closure algorithm \cite{ALLEN1984123} inspired by \cite{ning-etal-2018-joint} temporal constraints (Table~\ref{fig:figure1}). Applied after each annotation, this algorithm identifies and \textit{auto}-annotates unhandled pairs whose links can be transitively deduced from already annotated pairs, thereby reducing the number of pairs requiring \textit{manual} annotation. To optimize the algorithm's effectiveness, \App{} uses a prioritization strategy activated after each relation selection. For example, in Figure~\ref{fig:example}, once the pair \textit{`accident-collided'} is annotated as \textit{EQUAL}, the ideal next pair is \textit{`collided-damage'}. This choice maximizes the likelihood of automatically discovering a transitive relation, in this case, \textit{`accident-damage'}.\footnote{For more details, see Appendix~\ref{appx:prior-strategy}.} Before presenting the next pair for annotation, the tool ensures both completeness and consistency. In cases of contradicting relations, either in directly or transitively linked pairs—for example, scenario 7 in Table~\ref{tab:disc_temp}—the tool helps prevent errors such as mistakenly annotating the relation \(\{i, j\}\) as something other than \textit{EQUAL}. A notification highlighting the discrepancy is presented to guide the annotator in resolving the issue. When completeness and consistency are achieved, a notification is displayed indicating that no more pairs remain to be annotated.


\begin{figure}[t!]
\centering
\includegraphics[width=0.48\textwidth]{latex/figures/example1.png}
\caption{A simple example illustrating the prioritization strategy and automatic annotation of transitive relations. The tool sequentially presents the pairs \textit{`accident-collided'}, \textit{`collided-damage'}, and \textit{`damage-responded'} to the annotator, automatically annotating the relations \textit{`accident-damage'}, \textit{`accident-responded'}, and \textit{`collided-responded'}.}
\label{fig:example}
\end{figure}
%\caption{An illustration of \App{} steps: (1) Actual event selection; (2) Temporal relation annotation; (3) Coreference relation annotation; (4) Causal relation annotation.}


\subsection{Coreference Annotation}
\label{tool:coref}
The next step involves \emph{coreference} annotation ([3] in Figure~\ref{fig:figure1}). To reduce workload, this step only focuses on event-mention pairs labeled as concurrent in the previous step, as only these can potentially corefer. Here, annotators review a target event mention and its co-occurring mentions, alongside a graph visualization to monitor progress. They are required to identify which of the concurrent mentions corefer with the event mention in question, forming coreference clusters. Annotators then advances using a designated button (``Next Unhandled'') to the next unclustered event mention with co-occurring mentions. Upon completion of this step, event mentions not included in any cluster are marked as singleton clusters. Additionally, a discrepancy detection algorithm ensures consistency by notifying annotators of any event mention erroneously linked to multiple, non-coreferring clusters.
%Lastly, a relation graph visualization helps annotators track annotated relations, but unlike the previous step, it cannot be used to navigate to specific pairs.



\subsection{Causal Relation Annotation}
\label{tool:cause}
The final \emph{causal} relation annotation step ([4] in Figure~\ref{fig:figure1}) follows the EventStoryLine method \cite{caselli-vossen-2017-event}. Annotators examine an event mention within its context, alongside all events identified as preceding it in step [2], and determine which preceding events caused the event mention in focus. Similar to the previous steps, a relation graph visualization aids in tracking annotations, and a designated button allows annotators to navigate to the next event mention with at least one preceding event.

Unlike coreference and temporal relations, the EventStoryLine method treats causal relations as non-transitive and localized, alleviating the need for transitive and consistency checks.
After completing this step, annotators can run a completion check on the entire annotation, prompting the system to verify the annotations and, if any are missing, direct annotators to address the missing relations from previous steps.\footnote{For additional examples of \App{}, see Appendix~\ref{appx:additional_printscreens}.}



==> sections/acknowledgments.tex <==
\section*{Acknowledgments}


==> sections/ethical.tex <==
\section{Ethical Considerations}

